Generation and Applications of strong THz Fields driven by intense mid-IR Pulses

Although the THz spectral range experiences a tremendous grow of interest for at least two decades, it is still one of the least explored but most exciting areas to study light-matter interaction. Due to the small photon energy of THz radiation, it can propagate through non-conductive materials and resonantly interact with low-energy excitations, leading to a plethora of applications. The THz pulse is thereby primarily used as a probe while an optical pulse excites the material that is examined. In contrast, intense strong-field THz transients would allow on-demand control of the properties of matter. Current table-top THz sources remain rather weak, with the most promising being optical rectification (OR) in nonlinear crystals and two-color plasma filaments pumped by near-IR sources. While the former is mainly restricted by multi-photon absorption of the short wavelength driving pulse, causing crystal damage, the latter suffers from pump pulse scattering in dense plasma and limited laser field-asymmetry. These limitations can be surpassed with intense long wavelength driving pulses. Until recently, such high-power mid-IR sources were simply not available. In this work, we exploit the recently developed mid-IR optical parametric chirped pulse amplifier system to drive efficient THz generation in the organic crystal DAST by OR and in two-color plasma filaments, wherein we boost the optical- to THz conversion efficiency by almost an order of magnitude, compared to previous works with near-IR drivers. The intense THz source is further applied to heterostructure quantum dots without any field enhancing structures to investigate the pure quantum confined Stark effect. The possibility to manipulate optical properties of nano-scale semiconductors by direct THz radiation demonstrates the feasibility for an all-optical electro-absorption modulator with data rates in the range of Tbit/s.

==> Struktur/silben.tex <==
%%% Dokument für die Silbentrennung

\tolerance=2000                 % Zur Vermeidung von "overfull hbox"
\emergencystretch 20pt          % " besser als sloppy "


\hyphenation{Wis-sens-por-tal}


==> references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   Papers   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%% Applications and Intro %%%%%%%%%%%%%%%%%%%%%%%%%%%
@article{STRICKLAND:1985,
title = {Compression of amplified chirped optical pulses},
journal = {Optics Communications},
volume = {56},
number = {3},
pages = {219-221},
year = {1985},
issn = {0030-4018},
doi = {https://doi.org/10.1016/0030-4018(85)90120-8},
url = {https://www.sciencedirect.com/science/article/pii/0030401885901208},
author = {Donna Strickland and Gerard Mourou},
}

@article{Wilhelm:1997,
author = {T. Wilhelm and J. Piel and E. Riedle},
journal = {Opt. Lett.},
keywords = {Femtosecond pulses; Nonlinear optical crystals; Optical amplifiers; Phase matching; Ultrashort pulses; Visible light},
number = {19},
pages = {1494--1496},
publisher = {OSA},
title = {Sub-20-fs pulses tunable across the visible from a blue-pumped single-pass noncollinear parametric converter},
volume = {22},
month = {Oct},
year = {1997},
url = {http://opg.optica.org/ol/abstract.cfm?URI=ol-22-19-1494},
doi = {10.1364/OL.22.001494},
}

@article{Nichols:1923,
  title={{Joining the Infrared and Electric Wave Spectra}},
  author={E. F. Nichols, J. D. Tear},
  journal={Proceedings of the National Academy of Sciences of the United States of America},
  volume={9},
  number={6},
  pages={211--214},
  year={1923},
  url={https://pubmed.ncbi.nlm.nih.gov/16576702},
  doi={10.1073/pnas.9.6.211}
}

@article{Astro:2006,
	author = {{Dole, H.} and {Lagache, G.} and {Puget, J.-L.} and {Caputi, K. I.} and {Fern\'andez-Conde, N.} and {Le Floc'h, E.} and {Papovich, C.} and {P\'erez-Gonz\'alez, P. G.} and {Rieke, G. H.} and {Blaylock, M.}},
	title = {{The cosmic infrared background resolved by Spitzer - Contributions of mid-infrared galaxies to the far-infrared background}},
	DOI= "10.1051/0004-6361:20054446",
	url= "https://doi.org/10.1051/0004-6361:20054446",
	journal = {A\&A},
	year = 2006,
	volume = 451,
	number = 2,
	pages = "417-429",
}


@article{Flemming:1974,  
author={J. W. {Fleming}},  
journal={IEEE Transactions on Microwave Theory and Techniques},  
title={{High-Resolution Submillimeter-Wave Fourier-Transform Spectrometry of Gases}},   
year={1974},  
volume={22}, 
number={12},  
pages={1023-1025},
url={https://ieeexplore.ieee.org/abstract/document/1128419},
doi={10.1109/TMTT.1974.1128419},
}

@article{Hu:1995,
author = {B. B. Hu and M. C. Nuss},
journal = {Opt. Lett.},
number = {16},
pages = {1716--1718},
publisher = {OSA},
title = {{Imaging with terahertz waves}},
volume = {20},
month = {Aug},
year = {1995},
url = {http://ol.osa.org/abstract.cfm?URI=ol-20-16-1716},
doi = {10.1364/OL.20.001716},
}

@article{Nuss:1996, 
author={D. M. {Mittleman} and R. H. {Jacobsen} and M. C. {Nuss}}, 
journal={IEEE Journal of Selected Topics in Quantum Electronics}, 
title={{T-ray imaging}}, 
year={1996}, 
volume={2}, 
number={3}, 
pages={679--692},
url={https://ieeexplore.ieee.org/document/571768},
doi={10.1109/2944.571768}
}

@article{THzSpectroscopyBread:2002,
author = {Beard, Matthew C. and Turner, Gordon M. and Schmuttenmaer, Charles A.},
title = {{Terahertz Spectroscopy}},
journal = {The Journal of Physical Chemistry B},
volume = {106},
number = {29},
pages = {7146--7159},
year = {2002},
doi = {10.1021/jp020579i},
URL = {https://doi.org/10.1021/jp020579i},
}

@article{THzSpectroscopyMasayoshi:2007,
author = {Masayoshi Tonouchi},
title = {{Cutting-edge terahertz technology}},
journal = {Nature Photonics},
volume = {1},
number = {2},
pages = {97--105},
year = {2007},
doi = {10.1038/nphoton.2007.3},
URL = {https://doi.org/10.1038/nphoton.2007.3},
}



@article{THzSpectroscopyJepsen:2011,
author = {Jepsen, P.U. and Cooke, D.G. and Koch, M.},
title = {{Terahertz spectroscopy and imaging – Modern techniques and applications}},
journal = {Laser \& Photonics Reviews},
volume = {5},
number = {1},
pages = {124-166},
keywords = {Terahertz, spectroscopy, imaging, ultrafast.},
doi = {10.1002/lpor.201000011},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/lpor.201000011},
year = {2011}
}

@article{THzSpectroscopyBaxter:2011,
author = {Baxter, Jason B. and Guglietta, Glenn W.},
title = {{Terahertz Spectroscopy}},
journal = {Analytical Chemistry},
volume = {83},
number = {12},
pages = {4342-4368},
year = {2011},
doi = {10.1021/ac200907z},
URL = {https://doi.org/10.1021/ac200907z},
}

@article{ApplicationKolner:2008,
author={B. H. {Kolner} and R. A. {Buckles} and P. M. {Conklin} and R. P. {Scott}},
journal={IEEE Journal of Selected Topics in Quantum Electronics},
title={{Plasma Characterization With Terahertz Pulses}},
year={2008},
volume={14},
number={2},
pages={505-512},
doi={10.1109/JSTQE.2007.913395},
month={March},
}

@BOOK{THzHandbook:2015,
  TITLE = {{Handbook of Terahertz Technologies: Devices and Applications}},
  AUTHOR = {H.J. and Song T. Nagatsuma},
  YEAR = {2015},
  PUBLISHER = { Jenny Stanford Publishing},
URL = {https://doi.org/10.1201/b18381},  
  DOI = {10.1201/b18381},
}

@BOOK{SC_Optics:2012,
  TITLE = {{Semiconductor Optics}},
  AUTHOR = {Claus F. Klingshirn},
  YEAR = {2012},
  PUBLISHER = {Springer, Berlin, Heidelberg},
URL = {https://doi.org/10.1007/978-3-642-28362-8},  
  DOI = {10.1007/978-3-642-28362-8},
}

@book{Klimov:2010,
  title={{Nanocrystal Quantum Dots, Second Edition}},
  author={Klimov, V.I.},
  isbn={9781420079265},
  lccn={2009035684},
  series={Laser \& Optical Science \& Technology},
  url={https://books.google.at/books?id=BYIsyk3emCEC},
  year={2010},
  publisher={Taylor \& Francis}
}

@book{Landau:1977,
  title={Quantum Mechanics (Third Edition},
  author={L.D. Landau and E.M. Lifshitz},
  isbn={978-0-08-020940-1},
  url={https://www.sciencedirect.com/science/article/pii/B9780080209401500013},
  year={1977},
  publisher={Pergamon}
}


@book{Fluegge:1974,
  title={{Practical Quantum Mechanics}},
  author={Fl{\"u}gge, S.},
  isbn={9780387070506},
  lccn={74023732},
  series={Classics in mathematics},
  url={https://books.google.at/books?id=K0IsxQEACAAJ},
  year={1974},
  publisher={Springer Verlag}
}



@book{bastard:1988,
  title={{Wave Mechanics Applied to Semiconductor Heterostructures}},
  author={Bastard, G.},
  isbn={9780470217085},
  lccn={90047219},
  series={Monographies de physique},
  url={https://books.google.at/books?id=5rrvAAAAMAAJ},
  year={1988},
  publisher={Wiley}
}


@article{THzComSuen:2016,
	author = {Suen, Jonathan Y.},
	copyright = {Springer Science+Business Media New York},
	doi = {10.1007/s10762-016-0257-x},
	journal = {Journal of Infrared, Millimeter, and Terahertz Waves},
	keywords = {Terahertz communication; Satellite communication; Atmospheric propagation},
	language = {English},
	number = {7},
	pages = {615-639},
	title = {{Terabit-per-Second Satellite Links: a Path Toward Ubiquitous Terahertz Communication}},
	volume = {37},
	year = {2016},
}

@article{Baltuska:1992,
  title = {Controlling the Carrier-Envelope Phase of Ultrashort Light Pulses with Optical Parametric Amplifiers},
  author = {Baltu\ifmmode \check{s}\else \v{s}\fi{}ka, Andrius and Fuji, Takao and Kobayashi, Takayoshi},
  journal = {Phys. Rev. Lett.},
  volume = {88},
  issue = {13},
  pages = {133901},
  numpages = {4},
  year = {2002},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.88.133901},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.88.133901}
}

@article{RodamapDhillon:2017,
	doi = {10.1088/1361-6463/50/4/043001},
	url = {https://doi.org/10.1088/1361-6463/50/4/043001},
	year = 2017,
	month = {Jan},
	publisher = {{IOP} Publishing},
	volume = {50},
	number = {4},
	pages = {043001},
	author = {S S Dhillon and M S Vitiello and E H Linfield and A G Davies and Matthias C Hoffmann and John Booske and Claudio Paoloni and M Gensch and P Weightman and G P Williams and E Castro-Camus and D R S Cumming and F Simoens and I Escorcia-Carranza and J Grant and Stepan Lucyszyn and Makoto Kuwata-Gonokami and Kuniaki Konishi and Martin Koch and Charles A Schmuttenmaer and Tyler L Cocker and Rupert Huber and A G Markelz and Z D Taylor and Vincent P Wallace and J Axel Zeitler and Juraj Sibik and Timothy M Korter and B Ellison and S Rea and P Goldsmith and Ken B Cooper and Roger Appleby and D Pardo and P G Huggard and V Krozer and Haymen Shams and Martyn Fice and Cyril Renaud and Alwyn Seeds and Andreas Stöhr and Mira Naftaly and Nick Ridler and Roland Clarke and John E Cunningham and Michael B Johnston},
	title = {{The 2017 terahertz science and technology roadmap}},
	journal = {Journal of Physics D: Applied Physics},
}

@article{SalenNL_THz:2019,
title = {{Matter manipulation with extreme terahertz light: Progress in the enabling THz technology}},
journal = {Physics Reports},
volume = {836-837},
pages = {1-74},
year = {2019},
note = {{Matter manipulation with extreme terahertz light: Progress in the enabling THz technology}},
issn = {0370-1573},
doi = {https://doi.org/10.1016/j.physrep.2019.09.002},
url = {https://www.sciencedirect.com/science/article/pii/S0370157319302649},
author = {Peter Sal\'en and Martina Basini and Stefano Bonetti and J\'anos Hebling and Mikhail Krasilnikov and Alexey Y. Nikitin and Georgii Shamuilov and Zolt\'an Tibai and Vitali Zhaunerchyk and Vitaliy Goryashko}
}

@article{MedsApp:2019,
author ={Yu, Liu and Hao, Liu and Meiqiong, Tang and Jiaoqi, Huang and Wei, Liu and Jinying, Dong and Xueping, Chen and Weiling, Fu and Yang, Zhang},
title  ={{The medical application of terahertz technology in non-invasive detection of cells and tissues: opportunities and challenges}},
journal  ={RSC Adv.},
year  ={2019},
volume  ={9},
issue  ={17},
pages  ={9354-9363},
publisher  ={The Royal Society of Chemistry},
doi  ={10.1039/C8RA10605C},
url  ={http://dx.doi.org/10.1039/C8RA10605C},
}

@article{BioYang:2016,
title = {{Biomedical Applications of Terahertz Spectroscopy and Imaging}},
journal = {Trends in Biotechnology},
volume = {34},
number = {10},
pages = {810-824},
year = {2016},
issn = {0167-7799},
doi = {https://doi.org/10.1016/j.tibtech.2016.04.008},
url = {https://www.sciencedirect.com/science/article/pii/S0167779916300270},
author = {Xiang Yang and Xiang Zhao and Ke Yang and Yueping Liu and Yu Liu and Weiling Fu and Yang Luo},
}


@article{ExtremeTHz:2017,
author ={Zhang, Xi Cheng and Shkurinov, Alexander and Zhang, Yan},
title  ={Extreme terahertz science},
journal  ={Nature Photonics},
year  ={2017},
volume  ={11},
issue  ={1},
pages  ={16-18},
doi  ={10.1038/nphoton.2016.249},
url  ={https://doi.org/10.1038/nphoton.2016.249},
}

@article{Honey:2013,
author = {Maria Massaouti and Christina Daskalaki and Andrei Gorodetsky and Anastasios D. Koulouklidis and Stelios Tzortzakis},
title ={{Detection of Harmful Residues in Honey Using Terahertz Time-Domain Spectroscopy}},
journal = {Applied Spectroscopy},
volume = {67},
number = {11},
pages = {1264-1269},
year = {2013},
doi = {10.1366/13-07111},
url = {https://doi.org/10.1366/13-07111},
}

@article{DrugsPawar:2013,
title = {{Terahertz technology and its applications}},
journal = {Drug Invention Today},
volume = {5},
number = {2},
pages = {157-163},
year = {2013},
issn = {0975-7619},
doi = {https://doi.org/10.1016/j.dit.2013.03.009},
url = {https://www.sciencedirect.com/science/article/pii/S0975761913000264},
author = {Ashish Y. Pawar and Deepak D. Sonawane and Kiran B. Erande and Deelip V. Derle},
}

@Article{SalmonHindle:2018,
author ={Hindle, Francis and Kuuliala, Lotta and Mouelhi, Meriem and Cuisset, Arnaud and Bray, C\'edric and Vanwolleghem, Mathias and Devlieghere, Frank and Mouret, Ga\"{e}l and Bocquet, Robin},
title  ={{Monitoring of food spoilage by high resolution THz analysis}},
journal  ={Analyst},
year  ={2018},
volume  ={143},
issue  ={22},
pages  ={5536-5544},
publisher  ={The Royal Society of Chemistry},
doi  ={10.1039/C8AN01180J},
url  ={http://dx.doi.org/10.1039/C8AN01180J},
}

@article{Katayama:2012,
  title = {{Ferroelectric Soft Mode in a ${\mathrm{SrTiO}}_{3}$ Thin Film Impulsively Driven to the Anharmonic Regime Using Intense Picosecond Terahertz Pulses}},
  author = {Katayama, I. and Aoki, H. and Takeda, J. and Shimosato, H. and Ashida, M. and Kinjo, R. and Kawayama, I. and Tonouchi, M. and Nagai, M. and Tanaka, K.},
  journal = {Phys. Rev. Lett.},
  volume = {108},
  issue = {9},
  pages = {097401},
  numpages = {5},
  year = {2012},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.108.097401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.108.097401}
}

@article{Fleischer:2011,
  title = {{Molecular Orientation and Alignment by Intense Single-Cycle THz Pulses}},
  author = {Fleischer, Sharly and Zhou, Yan and Field, Robert W. and Nelson, Keith A.},
  journal = {Phys. Rev. Lett.},
  volume = {107},
  issue = {16},
  pages = {163603},
  numpages = {5},
  year = {2011},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.107.163603},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.107.163603}
}

@article{SpinChoi:2020,
author = {Choi,B. C.  and Rudge,J.  and Jordan,K.  and Genet,T. },
title = {{Terahertz excitation of spin dynamics in ferromagnetic thin films incorporated in metallic spintronic-THz-emitter}},
journal = {Applied Physics Letters},
volume = {116},
number = {13},
pages = {132406},
year = {2020},
doi = {10.1063/1.5143133},
URL = {https://doi.org/10.1063/1.5143133},
}

@article{Razzari:2009,
  title = {{Nonlinear ultrafast modulation of the optical absorption of intense few-cycle terahertz pulses in $n$-doped semiconductors}},
  author = {Razzari, L. and Su, F. H. and Sharma, G. and Blanchard, F. and Ayesheshim, A. and Bandulet, H.-C. and Morandotti, R. and Kieffer, J.-C. and Ozaki, T. and Reid, M. and Hegmann, F. A.},
  journal = {Phys. Rev. B},
  volume = {79},
  issue = {19},
  pages = {193204},
  numpages = {4},
  year = {2009},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.79.193204},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.79.193204}
}

@article{Ham:2017,
author = {Hamm,Peter  and Meuwly,Markus  and Johnson,Steve L.  and Beaud,Paul  and Staub,Urs },
title = {{Perspective: THz-driven nuclear dynamics from solids to molecules}},
journal = {Structural Dynamics},
volume = {4},
number = {6},
pages = {061601},
year = {2017},
doi = {10.1063/1.4992050},
URL = {https://doi.org/10.1063/1.4992050},
eprint = {https://doi.org/10.1063/1.4992050},
}

@ARTICLE{Razzari:2010,
author={Sharma, G. and Razzari, L. and Su, F. H. and Blanchard, F. and Ayesheshim, A. and Cocker, T. L. and Titova, L. V. and Bandulet, H. C. and Ozaki, T. and Kieffer, J.-C. and Morandotti, R. and Reid, M. and Hegmann, F. A.},
journal={IEEE Photonics Journal}, 
title={{Time-Resolved Terahertz Spectroscopy of Free Carrier Nonlinear Dynamics in Semiconductors}}, 
year={2010},
volume={2},
number={4},
pages={578-592},
doi={10.1109/JPHOT.2010.2050873},
}

@article{Phonons:2010,
author = {Manceau,J.-M.  and Loukakos,P. A.  and Tzortzakis,S. },
title = {{Direct acoustic phonon excitation by intense and ultrashort terahertz pulses}},
journal = {Applied Physics Letters},
volume = {97},
number = {25},
pages = {251904},
year = {2010},
doi = {10.1063/1.3529466},
URL = {https://doi.org/10.1063/1.3529466},
eprint = {https://doi.org/10.1063/1.3529466}
}

@article{IntenseHafez:2016,
	doi = {10.1088/2040-8978/18/9/093004},
	url = {https://doi.org/10.1088/2040-8978/18/9/093004},
	year = 2016,
	month = {aug},
	publisher = {{IOP} Publishing},
	volume = {18},
	number = {9},
	pages = {093004},
	author = {H A Hafez and X Chai and A Ibrahim and S Mondal and D F{\'{e}}rachou and X Ropagnol and T Ozaki},
	title = {{Intense terahertz radiation and their applications}},
	journal = {Journal of Optics},
}

@article{Superconductivity:2012,
  title = {{Nonequilibrium BCS State Dynamics Induced by Intense Terahertz Pulses in a Superconducting NbN Film}},
  author = {Matsunaga, Ryusuke and Shimano, Ryo},
  journal = {Phys. Rev. Lett.},
  volume = {109},
  issue = {18},
  pages = {187002},
  numpages = {5},
  year = {2012},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.109.187002},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.109.187002}
}

@article{Baierl:2016,
  title = {{Nonlinear spin control by terahertz-driven anisotropy fields}},
  author = {Baierl, S. and Hohenleutner, M. and Kampfrath, T. and Zvezdin, A. K.and Kimel, A. V. and Huber, R. and Mikhaylovskiy, R. V.},
  journal = {Nature Photonics},
  volume = {10},
  issue = {11},
  pages = {715--718},
  year = {2016},
  doi = {10.1038/nphoton.2016.181},
  url = {https://doi.org/10.1038/nphoton.2016.181}
}

@ARTICLE{Eacc_Nanni:2015,
    author = {{Nanni}, Emilio A. and {Huang}, Wenqian R. and {Hong}, Kyung-Han and {Ravi}, Koustuban and {Fallahi}, Arya and {Moriena}, Gustavo and {Dwayne Miller}, R.~J. and {K{\"a}rtner}, Franz X.},
    title = {{Terahertz-driven linear electron acceleration}},
    journal = {Nature Communications},
    keywords = {Physics - Accelerator Physics},
    year = {2015},
    volume = {6},
    pages = {8486},
    doi = {10.1038/ncomms9486},
    url = {https://ui.adsabs.harvard.edu/abs/2015NatCo...6.8486N},
}

@ARTICLE{Eacc_Zhang:2018,
    author = {Zhang, Dongfang and Fallahi, Arya and Hemmer, Michael and Wu, Xiaojun and Fakhari, Moein and {Hua}, Yi and Cankaya, Huseyin and Calendron, Anne-Laure and Zapata, Luis E. and Matlis, Nicholas H. and K{\"a}rtner, Franz X.},
    title = {Segmented terahertz electron accelerator and manipulator {(STEAM)}},
    journal = {Nature Photonics},
    year = {2018},
    volume = {12},
    number = {6},
    pages = {336-342},
    doi = {10.1038/s41566-018-0138-z},
    url = {https://ui.adsabs.harvard.edu/abs/2018NaPho..12..336Z},
}

@article{Grishunin:2017,
  title = {{THz Electric Field-Induced Second Harmonic Generation in Inorganic Ferroelectric}},
  author = {Grishunin, Kirill A. and Ilyin, Nikita A. and Sherstyuk, Natalia E. and Mishina, Elena D. and Kimel, Alexey and Mukhortov, Vladimir M. and Ovchinnikov, Andrey V. and Chefonov, Oleg V. and Agranat, Mikhail B.},
  journal = {Scientific Reports},
  volume = {7},
  issue = {1},
  pages = {687},
  year = {2017},
  doi = {10.1038/s41598-017-00704-9},
  url = {https://doi.org/10.1038/s41598-017-00704-9}
}

%%%%%%%%%%%%%%%%%%%%%%%%%% THz sources and Intro%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Tasos:2020,
  title = {{Observation of extremely efficient terahertz generation from mid-infrared two-color laser filaments}},
  author = {Koulouklidis, Anastasios D. and Gollner, Claudia and Shumakova, Valentina and Fedorov, Vladimir Yu. and Pug\v{z}lys, Audrius and Baltu\v{s}ka, Andrius and Tzortzakis, Stelios},
  journal = {Nature Communications},
  volume = {11},
  issue = {1},
  pages = {292},
  year = {2020},
  doi = {10.1038/s41467-019-14206-x},
  url = {https://doi.org/10.1038/s41467-019-14206-x}
}

@article{Gollner:2021,
author = {Gollner,Claudia  and Shalaby,Mostafa  and Brodeur,Corinne  and Astrauskas,Ignas  and Jutas,Rokas  and Constable,Evan  and Bergen,Lorenz  and Baltu\v{s}ka, Andrius  and Pug\v{z}lys, Audrius },
title = {{Highly efficient THz generation by optical rectification of mid-IR pulses in DAST}},
journal = {APL Photonics},
volume = {6},
number = {4},
pages = {046105},
year = {2021},
doi = {10.1063/5.0037235},
URL = {https://doi.org/10.1063/5.0037235},
eprint = {https://doi.org/10.1063/5.0037235}
}

@article{SLAC:2013,
author = {Wu,Ziran  and Fisher,Alan S.  and Goodfellow,John  and Fuchs,Matthias  and Daranciang,Dan  and Hogan,Mark  and Loos,Henrik  and Lindenberg,Aaron },
title = {{Intense terahertz pulses from SLAC electron beams using coherent transition radiation}},
journal = {Review of Scientific Instruments},
volume = {84},
number = {2},
pages = {022701},
year = {2013},
doi = {10.1063/1.4790427},
URL = {https://doi.org/10.1063/1.4790427},
eprint = {https://doi.org/10.1063/1.4790427}
}

@article{FACET:2011,
author = {Daranciang,Dan  and Goodfellow,John  and Fuchs,Matthias  and Wen,Haidan  and Ghimire,Shambhu  and Reis,David A.  and Loos,Henrik  and Fisher,Alan S.  and Lindenberg,Aaron M. },
title = {{Single-cycle terahertz pulses with > \SI{0.2}{V/\angstrom} field amplitudes via coherent transition radiation}},
journal = {Applied Physics Letters},
volume = {99},
number = {14},
pages = {141117},
year = {2011},
doi = {10.1063/1.3646399},
URL = {https://doi.org/10.1063/1.3646399},
eprint = {https://doi.org/10.1063/1.3646399}
}

@article{FLASH:2008,
author = {M. Gensch and L. Bittner and A. Chesnov and H. Delsim-Hashemi and M. Drescher and B. Faatz and J. Feldhaus and U. Fruehling and G.A. Geloni and Ch. Gerth and O. Grimm and U. Hahn and M. Hesse and S. Kapitzki and V. Kocharyan and O. Kozlov and E. Matyushevsky and N. Morozov and D. Petrov and E. Ploenjes and M. Roehling and J. Rossbach and E.L. Saldin and B. Schmidt and P. Schmueser and E.A. Schneidmiller and E. Syresin and A. Willner and M.V. Yurkov},
title = {{New infrared undulator beamline at FLASH}},
journal = {Infrared Physics \& Technology},
volume = {51},
number = {5},
pages = {423-425},
year = {2008},
note = {4th International Workshop on Infrared Microscopy and Spectroscopy with Accelerator-Based Sources},
issn = {1350-4495},
doi = {https://doi.org/10.1016/j.infrared.2007.12.032},
url = {https://www.sciencedirect.com/science/article/pii/S1350449507001193},
}

@article{FLASH:2016,
author = {Awari, N. and Nicoletti, D. and Kaiser, S. and Laplace, Y. and Rajasekaran, S. and Zhang, L. and Winnerl, S. and Schneider, H. and Schay, G. and Lorincz, I. and Rauscher, A. A. and Radu, I. and M\"{a}hrlein, S. and Kim, T. H. and Lee, J. S. and Kampfrath, T. and Wall, S. and Heberle, J. and Malnasi-Csizmadia, A. and Steiger, A. and M\"{u}ller, A. S. and Helm, M. and Schramm, U. and Cowan, T. and Michel, P. and Cavalleri, A. and Fisher, A. S. and Stojanovic, N. and Gensch, M.},
title = {{High-Field High-Repetition-Rate Sources for the Coherent THz Control of Matter}},
journal = {Scientific Reports},
volume = {6},
pages = {22256},
year = {2016},
issn = {1},
doi = {10.1038/srep22256},
url = {https://doi.org/10.1038/srep22256},
}


@Article{Review:2021,
AUTHOR = {Zhu, Xing and Bacon, David R. and Madéo, Julien and Dani, Keshav M.},
TITLE ={{High Field Single- to Few-Cycle THz Generation with Lithium Niobate}},
JOURNAL = {Photonics},
VOLUME = {8},
YEAR = {2021},
NUMBER = {6},
ARTICLE-NUMBER = {183},
URL = {https://www.mdpi.com/2304-6732/8/6/183},
ISSN = {2304-6732},
DOI = {10.3390/photonics8060183},
} 
@article{ORefficiencyHuang:2013,
author = {Shu-Wei Huang and Eduardo Granados and Wenqian Ronny Huang and Kyung-Han Hong and Luis E. Zapata and Franz X. K\"{a}rtner},
journal = {Opt. Lett.},
number = {5},
pages = {796--798},
publisher = {OSA},
title = {{High conversion efficiency, high energy terahertz pulses by optical rectification in cryogenically cooled lithium niobate}},
volume = {38},
month = {Mar},
year = {2013},
url = {http://ol.osa.org/abstract.cfm?URI=ol-38-5-796},
doi = {10.1364/OL.38.000796},
}

@article{LiNbZhang:2021,
author = {Zhang, Baolong and Ma, Zhenzhe and Ma, Jinglong and Wu, Xiaojun and Ouyang, Chen and Kong, Deyin and Hong, Tianshu and Wang, Xuan and Yang, Peidi and Chen, Liming and Li, Yutong and Zhang, Jie},
title = {{1.4-mJ High Energy Terahertz Radiation from Lithium Niobates}},
journal = {Laser \& Photonics Reviews},
volume = {15},
number = {3},
pages = {2000295},
keywords = {lithium niobate, nonlinear optics, strong field, Terahertz},
doi = {https://doi.org/10.1002/lpor.202000295},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/lpor.202000295},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/lpor.202000295},
year = {2021}
}

@article{ApplicationGreenland:2010,
author = {Greenland, P. T. and Lynch, S. A. and van der Meer, A. F. G. and Murdin, B. N. and Pidgeon, C. R. and Redlich, B. and Vinh, N. Q. and Aeppli, G.},
title = {{Coherent control of Rydberg states in silicon}},
journal = {Nature},
volume = {465},
pages = {1057 -- 1061},
year = {2010},
doi = {10.1038/nature09112},
url = {https://doi.org/10.1038/nature09112},
}

@article{DSTMSVicario09:2014,
author = {C. Vicario and A. V. Ovchinnikov and S. I. Ashitkov and M. B. Agranat and V. E. Fortov and C. P. Hauri},
journal = {Opt. Lett.},
number = {23},
pages = {6632--6635},
publisher = {OSA},
title = {Generation of 0.9-{mJ} {THz} pulses in {DSTMS} pumped by a {Cr:Mg2SiO4} laser},
volume = {39},
month = {Dec},
year = {2014},
url = {http://ol.osa.org/abstract.cfm?URI=ol-39-23-6632},
doi = {10.1364/OL.39.006632},
}

@article{DASTHauri:2011,
author = {Hauri,Christoph P.  and Ruchert,Clemens  and Vicario,Carlo  and Ardana,Fernando },
title = {Strong-field single-cycle {THz} pulses generated in an organic crystal},
journal = {Applied Physics Letters},
volume = {99},
number = {16},
pages = {161116},
year = {2011},
doi = {10.1063/1.3655331},
URL = {https://doi.org/10.1063/1.3655331},
}

@article{DASTVicario:2015,
author = {C. Vicario and M. Jazbinsek and A. V. Ovchinnikov and O. V. Chefonov and S. I. Ashitkov and M. B. Agranat and C. P. Hauri},
journal = {Opt. Express},
number = {4},
pages = {4573--4580},
publisher = {OSA},
title = {High efficiency {THz} generation in {DSTMS}, {DAST} and {OH1} pumped by {Cr:forsterite} laser},
volume = {23},
month = {Feb},
year = {2015},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-23-4-4573},
doi = {10.1364/OE.23.004573},
}

@article{BulletShalaby:2015,
  title = {{Demonstration of a low-frequency three-dimensional terahertz bullet with extreme brightness}},
  author = {Shalaby, Mostafa and Hauri, Christoph P.},
  journal = {Nature Communications},
  volume = {6},
  issue = {1},
  pages = {5976},
  year = {2015},
  doi = {10.1038/ncomms6976},
  url = {https://doi.org/10.1038/ncomms6976}
}

@article{Monoszlai:2013,
author = {B. Monoszlai and C. Vicario and M. Jazbinsek and C. P. Hauri},
journal = {Opt. Lett.},
keywords = {Laser damage; Ultrafast lasers; Nonlinear optics, materials; Nonlinear optics, parametric processes; Optical nonlinearities in organic materials; Ultrafast nonlinear optics; Laser energy; Optical amplifiers; Optical rectification; Phase velocity; Terahertz generation; Ti:sapphire lasers},
number = {23},
pages = {5106--5109},
publisher = {OSA},
title = {{High-energy terahertz pulses from organic crystals: DAST and DSTMS pumped at Ti:sapphire wavelength}},
volume = {38},
month = {Dec},
year = {2013},
url = {http://ol.osa.org/abstract.cfm?URI=ol-38-23-5106},
doi = {10.1364/OL.38.005106},

}

@article{PlasmaWidth:2013,
	doi = {10.1088/1367-2630/15/7/075002},
	url = {https://doi.org/10.1088/1367-2630/15/7/075002},
	year = 2013,
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {15},
	number = {7},
	pages = {075002},
	author = {T I Oh and Y S You and N Jhajj and E W Rosenthal and H M Milchberg and K Y Kim},
	title = {{Intense terahertz generation in two-color laser filamentation: energy scaling with terawatt laser systems}},
	journal = {New Journal of Physics}
}

@article{PlasmaWidthKim:2008,
	doi = {10.1038/nphoton.2008.153},
	url = {https://doi.org/10.1038/nphoton.2008.153},
	year = 2008,
	volume = {2},
	issue = {10},
	pages = {605--609},
	author = {Kim, K. Y. and Taylor, A. J. and Glownia, J. H. and Rodriguez, G.},
	title = {{Coherent control of terahertz supercontinuum generation in ultrafast laser-gas interactions}},
	journal = {Nature Photonics}
}

@article{Nguyen:2019,
author = {A. Nguyen and K. J. Kaltenecker and J.-C. Delagnes and B. Zhou and E. Cormier and N. Fedorov and R. Bouillaud and D. Descamps and I. Thiele and S. Skupin and P. U. Jepsen and L. Berg\'{e}},
journal = {Opt. Lett.},
number = {6},
pages = {1488--1491},
publisher = {OSA},
title = {Wavelength scaling of terahertz pulse energies delivered by two-color air plasmas},
volume = {44},
month = {Mar},
year = {2019},
url = {http://www.osapublishing.org/ol/abstract.cfm?URI=ol-44-6-1488},
doi = {10.1364/OL.44.001488},
}

@article{PlasmaKuk:2016,
author = {Kuk,D.  and Yoo,Y. J.  and Rosenthal,E. W.  and Jhajj,N.  and Milchberg,H. M.  and Kim,K. Y. },
title = {{Generation of scalable terahertz radiation from cylindrically focused two-color laser pulses in air}},
journal = {Applied Physics Letters},
volume = {108},
number = {12},
pages = {121106},
year = {2016},
doi = {10.1063/1.4944843},
URL = {https://doi.org/10.1063/1.4944843},
eprint = { https://doi.org/10.1063/1.4944843}
}

@article{PlasmaOhKim:2013,
author = {Oh,T. I.  and You,Y. S.  and Jhajj,N.  and Rosenthal,E. W.  and Milchberg,H. M.  and Kim,K. Y. },
title = {{Scaling and saturation of high-power terahertz radiation generation in two-color laser filamentation}},
journal = {Applied Physics Letters},
volume = {102},
number = {20},
pages = {201113},
year = {2013},
doi = {10.1063/1.4807790},
URL = {https://doi.org/10.1063/1.4807790},
eprint = {https://doi.org/10.1063/1.4807790}
}

@INPROCEEDINGS{KimProceeding:2020,
author={Ki-Yong Kim},
booktitle={{4th Asia-Pacific Conference on Plasma Physics}}, 
title={High power terahertz generation from laser-plasma interactions}, 
year={2020},
volume={},
number={},
pages={PL-34 AAPPS-DPP2020},
doi={}
}

@article{LongWLplasma:2013,
  title = {{Wavelength Scaling of Terahertz Generation by Gas Ionization}},
  author = {Clerici, Matteo and Peccianti, Marco and Schmidt, Bruno E. and Caspani, Lucia and Shalaby, Mostafa and Gigu\`ere, Mathieu and Lotti, Antonio and Couairon, Arnaud and L\'egar\'e, Fran\ifmmode \mbox{\c{c}}\else \c{c}\fi{}ois and Ozaki, Tsuneyuki and Faccio, Daniele and Morandotti, Roberto},
  journal = {Phys. Rev. Lett.},
  volume = {110},
  issue = {25},
  pages = {253901},
  numpages = {5},
  year = {2013},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.110.253901},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.110.253901}
}

@article{StrongFieldFulop:2020,
author = {Fülöp, József András and Tzortzakis, Stelios and Kampfrath, Tobias},
title = {{Laser-Driven Strong-Field Terahertz Sources}},
journal = {Advanced Optical Materials},
volume = {8},
number = {3},
pages = {1900681},
keywords = {optical rectification, plasma-based terahertz sources, spintronic emitters, strong-field terahertz–matter interactions, terahertz pulses},
doi = {https://doi.org/10.1002/adom.201900681},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/adom.201900681},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/adom.201900681},
year = {2020}
}

@ARTICLE{SOTAplasma:2017,
author={Yoo, Yung-Jun and Kuk, Donghoon and Zhong, Zheqiang and Kim, Ki-Yong},
journal={IEEE Journal of Selected Topics in Quantum Electronics}, 
title={{Generation and Characterization of Strong Terahertz Fields From kHz Laser Filamentation}}, 
year={2017},
volume={23},
number={4},
pages={1-7},
doi={10.1109/JSTQE.2016.2644259}
}

@article{Fulop:2014,
author = {J. A. F\"{u}l\"{o}p and Z. Ollmann and Cs. Lombosi and C. Skrobol and S. Klingebiel and L. P\'{a}lfalvi and F. Krausz and S. Karsch and J. Hebling},
journal = {Opt. Express},
keywords = {Lithium niobate; Nonlinear optics; Spectroscopy, teraherz ; Diode pumped lasers; Electric fields; Lithium niobate; Optical rectification; Pulse generation; Terahertz generation},
number = {17},
pages = {20155--20163},
publisher = {OSA},
title = {{Efficient generation of THz pulses with 0.4 mJ energy}},
volume = {22},
month = {Aug},
year = {2014},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-22-17-20155},
doi = {10.1364/OE.22.020155},
}

@article {THz55mJ:2019,
	author = {Liao, Guoqian and Li, Yutong and Liu, Hao and Scott, Graeme G. and Neely, David and Zhang, Yihang and Zhu, Baojun and Zhang, Zhe and Armstrong, Chris and Zemaityte, Egle and Bradford, Philip and Huggard, Peter G. and Rusby, Dean R. and McKenna, Paul and Brenner, Ceri M. and Woolsey, Nigel C. and Wang, Weimin and Sheng, Zhengming and Zhang, Jie},
	title = {{Multimillijoule coherent terahertz bursts from picosecond laser-irradiated metal foils}},
	volume = {116},
	number = {10},
	pages = {3994--3999},
	year = {2019},
	doi = {10.1073/pnas.1815256116},
	publisher = {National Academy of Sciences},
	issn = {0027-8424},
	URL = {https://www.pnas.org/content/116/10/3994},
	eprint = {https://www.pnas.org/content/116/10/3994.full.pdf},
	journal = {Proceedings of the National Academy of Sciences}
}

@article{Herzer:2018,
	doi = {10.1088/1367-2630/aaada0},
	url = {https://doi.org/10.1088/1367-2630/aaada0},
	year = 2018,
	month = {jun},
	publisher = {{IOP} Publishing},
	volume = {20},
	number = {6},
	pages = {063019},
	author = {S Herzer and A Woldegeorgis and J Polz and A Reinhard and M Almassarani and B Beleites and F Ronneberger and R Grosse and G G Paulus and U Hübner and T May and A Gopal},
	title = {An investigation on {THz} yield from laser-produced solid density plasmas at relativistic laser intensities},
	journal = {New Journal of Physics},
}

@inproceedings{Vulcan:1999,
author = {Colin N. Danson and Ric M. Allott and S. Angood and G. Booth and J. L. Collier and A. R. Damerell and Christopher B. Edwards and P. S. Flintoff and J. Govans and S. Hancock and P. Hatton and S. J. Hawkes and M. H. R. Hutchinson and Michael H. Key and C. Hernandez-Gomez and John Leach and W. Lester and David Neely and Peter A. Norreys and M. M. Notley and David A. Pepler and C. J. Reason and D. A. Rodkiss and Ian N. Ross and W. T. Toner and M. Trentelman and J. A. Walczak and R. A. Wellstood and T. B. Winstone and R. W. W. Wyatt and B. E. Wyborn},
title = {{Focused intensities of 1020 Wcm-2 with the upgraded Vulcan CPA interaction facility}},
volume = {3492},
booktitle = {Third International Conference on Solid State Lasers for Application to Inertial Confinement Fusion},
editor = {W. Howard Lowdermilk},
organization = {International Society for Optics and Photonics},
publisher = {SPIE},
pages = {82 -- 93},
year = {1999},
doi = {10.1117/12.354151},
URL = {https://doi.org/10.1117/12.354151}
}

@article{Vulcan:2006,
	author = {{C. Hernandez-Gomez} and {P.A. Brummitt} and {D.J. Canny} and {R.J. Clarke} and {J. Collier} and {C.N. Danson} and {A.M. Dunne} and {B. Fell} and {A.J. Frackiewicz} and {S. Hancock} and {S. Hawkes} and {R. Heathcote} and {P. Holligan} and {M.H.R. Hutchinson} and {A. Kidd} and {W.J. Lester} and {I.O. Musgrave} and {D. Neely} and {D.R. Neville} and {P.A. Norreys} and {D.A. Pepler} and {C.J. Reason} and {W. Shaikh} and {T.B. Winstone} and {B.E. Wyborn}},
	title = {Vulcan petawatt-operation and development},
	DOI= "10.1051/jp4:2006133114",
	url= "https://doi.org/10.1051/jp4:2006133114",
	journal = {J. Phys. IV France},
	year = 2006,
	volume = 133,
	pages = "555-559",
	month = "",
}

@INPROCEEDINGS{Vulcan:2019,
author={Archipovaite, Giedre and Galletti, Mario and Oliveira, Pedro and Ahmad, Munadi and Clarke, Rob and Neely, David and Booth, Nicola and Heathcote, Rob and Galimberti, Marco and Musgrave, Ian and Hernandez-Gomez, Cristina},
booktitle={2019 Conference on Lasers and Electro-Optics Europe   European Quantum Electronics Conference (CLEO/Europe-EQEC)}, 
title={Progress of the Development of New Vulcan PW OPCPA Beamline}, 
year={2019},
volume={},
number={},
pages={1-1},
doi={10.1109/CLEOE-EQEC.2019.8872259},
}


@article{FLASH:2013,
	doi = {10.1088/0953-4075/46/19/192001},
	url = {https://doi.org/10.1088/0953-4075/46/19/192001},
	year = 2013,
	month = {sep},
	publisher = {{IOP} Publishing},
	volume = {46},
	number = {19},
	pages = {192001},
	author = {Nikola Stojanovic and Markus Drescher},
	title = {{Accelerator- and laser-based sources of high-field terahertz pulses}},
	journal = {Journal of Physics B: Atomic, Molecular and Optical Physics},
}

@article{SR:1954,
  title = {Suppression of Coherent Radiation by Electrons in a Synchrotron},
  author = {Nodvick, John S. and Saxon, David S.},
  journal = {Phys. Rev.},
  volume = {96},
  issue = {1},
  pages = {180--184},
  numpages = {0},
  year = {1954},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.96.180},
  url = {https://link.aps.org/doi/10.1103/PhysRev.96.180}
}

@article{SR:1991,
  title = {Multiparticle coherence calculations for synchrotron-radiation emission},
  author = {Hirschmugl, Carol J. and Sagurton, Michael and Williams, Gwyn P.},
  journal = {Phys. Rev. A},
  volume = {44},
  issue = {2},
  pages = {1316--1320},
  numpages = {0},
  year = {1991},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.44.1316},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.44.1316}
}

@article{SR:2002,
  title = {High-power terahertz radiation from relativistic electrons},
  author = {Carr, G. L. and Martin, Michael C. and McKinney, Wayne R. and Jordan, K. and Neil, George R. and Williams, G. P.},
  journal = {Nature},
  volume = {420},
  issue = {6912},
  pages = {153--156},
  numpages = {4},
  year = {2002},
  month = {Sep},
  doi = {10.1038/nature01175},
  url = {https://doi.org/10.1038/nature01175}
}



@article{Mak:2019,
	doi = {10.1088/1361-6633/aafa35},
	url = {https://doi.org/10.1088/1361-6633/aafa35},
	year = {2019},
	month = {Jan},
	publisher = {{IOP} Publishing},
	volume = {82},
	number = {2},
	pages = {025901},
	author = {Alan Mak and Georgii Shamuilov and Peter Sal{\'{e}}n and David Dunning and J{\'{a}}nos Hebling and Yuichiro Kida and Ryota Kinjo and Brian W J McNeil and Takashi Tanaka and Neil Thompson and Zolt{\'{a}}n Tibai and György T{\'{o}}th and Vitaliy Goryashko},
	title = {Attosecond single-cycle undulator light: a review},
	journal = {{Reports on Progress in Physics}},
}

@article{Green:2016,
	doi = {10.1038/srep22256},
	url = {https://doi.org/10.1038/srep22256},
	year = {2016},
	month = {Feb},
	publisher = {Nature publishing group},
	volume = {6},
	number = {1},
	pages = {22256},
	author = {Green, B. and Kovalev, S. and Asgekar, V. and Geloni, G. and Lehnert, U. and Golz, T. and Kuntzsch, M. and Bauer, C. and Hauser, J. and Voigtlaender, J. and Wustmann, B. and Koesterke, I. and Schwarz, M. and Freitag, M. and Arnold, A. and Teichert, J. and Justus, M. and Seidel, W. and Ilgner, C. and Awari, N. and Nicoletti, D. and Kaiser, S. and Laplace, Y. and Rajasekaran, S. and Zhang, L. and Winnerl, S. and Schneider, H. and Schay, G. and Lorincz, I. and Rauscher, A. A. and Radu, I. and Mährlein, S. and Kim, T. H. and Lee, J. S. and Kampfrath, T. and Wall, S. and Heberle, J. and Malnasi-Csizmadia, A. and Steiger, A. and Müller, A. S. and Helm, M. and Schramm, U. and Cowan, T. and Michel, P. and Cavalleri, A. and Fisher, A. S. and Stojanovic, N. and Gensch, M.
},
	title = {{High-Field High-Repetition-Rate Sources for the Coherent THz Control of Matter}},
	journal = {Scientific Reports},
}

@INPROCEEDINGS{FLASH:2019,
  author={Pan, Rui and Zapolnova, Ekaterina and Stojanovic, Nikola},
  booktitle={2019 44th International Conference on Infrared, Millimeter, and Terahertz Waves (IRMMW-THz)}, 
  title={{Ultrafast High-Field THz beamline at X-ray FEL}}, 
  year={2019},
  volume={},
  number={},
  pages={1-1},
  doi={10.1109/IRMMW-THz.2019.8873919}}

@article{CTR:2003,
author = {Zheng,Jian  and Tanaka,K. A.  and Miyakoshi,T.  and Kitagawa,Y.  and Kodama,R.  and Kurahashi,T.  and Yamanaka,T. },
title = {Theoretical study of transition radiation from hot electrons generated in the laser–solid interaction},
journal = {Physics of Plasmas},
volume = {10},
number = {7},
pages = {2994-3003},
year = {2003},
doi = {10.1063/1.1576388},
URL = {https://doi.org/10.1063/1.1576388},
eprint = {https://doi.org/10.1063/1.1576388},
}

@book{CTRbook:1972,
    author    = {M. L. Ter-Mikaelian},
    title     = {{High-energy electromagnetic processes in condensed media}},
    year      = {1972},
    publisher = {Wiley-Interscience},
    address   = {New York}
}

@article{pca:2017,
author = {Nathan   M. Burford and Magda   O. El-Shenawee},
title = {{Review of terahertz photoconductive antenna technology}},
volume = {56},
journal = {Optical Engineering},
number = {1},
publisher = {SPIE},
pages = {1 -- 20},
keywords = {terahertz, photoconductive antenna, spectroscopy, Terahertz radiation, Principal component analysis, Antennas, Electrodes, Gallium arsenide, Terahertz technology, Plasmonics, Nanostructures, Signal to noise ratio, Sensors},
year = {2017},
doi = {10.1117/1.OE.56.1.010901},
URL = {https://doi.org/10.1117/1.OE.56.1.010901}
}

@article{Ropagnol:2016,
author = {X. Ropagnol and M. Khorasaninejad and M. Raeiszadeh and S. Safavi-Naeini and M. Bouvier and C. Y. C\^{o}t\'{e} and A. Laram\'{e}e and M. Reid and M. A. Gauthier and T. Ozaki},
journal = {Opt. Express},
keywords = {Infrared, far; Ultrafast nonlinear optics; Spectroscopy, teraherz ; Switching ; Corona discharges; Electric fields; High harmonic generation; Nonlinear absorption; Terahertz generation; Ti:sapphire lasers},
number = {11},
pages = {11299--11311},
publisher = {OSA},
title = {Intense THz Pulses with large ponderomotive potential generated from large aperture photoconductive antennas},
volume = {24},
month = {May},
year = {2016},
url = {http://www.osapublishing.org/oe/abstract.cfm?URI=oe-24-11-11299},
doi = {10.1364/OE.24.011299},
}

@ARTICLE{Ropagnol:2017,
author={Ropagnol, Xavier and Chai, Xin and Raeis-Zadeh, S. Mohsen and Safavi-Naeini, Safieddin and Kirouac-Turmel, Marie and Bouvier, Marcel and Côté, Christian-Yves and Reid, Matt and Gauthier, Marc Andre and Ozaki, Tsuneyuki},
journal={IEEE Journal of Selected Topics in Quantum Electronics}, 
title={{Influence of Gap Size on Intense THz Generation From ZnSe Interdigitated Large Aperture Photoconductive Antennas}}, 
year={2017},
volume={23},
number={4},
pages={1-8},
doi={10.1109/JSTQE.2017.2662658},
}

@article{Singh:21,
author = {Abhishek Singh and Jiang Li and Alexej Pashkin and Rakesh Rana and Stephan Winnerl and Manfred Helm and Harald Schneider},
journal = {Opt. Express},
keywords = {Electric fields; Electromagnetic radiation; Laser systems; Optical rectification; Terahertz spectroscopy; Ti:sapphire lasers},
number = {13},
pages = {19920--19927},
publisher = {OSA},
title = {{High-field THz pulses from a GaAs photoconductive emitter for non-linear THz studies}},
volume = {29},
month = {Jun},
year = {2021},
url = {http://www.osapublishing.org/oe/abstract.cfm?URI=oe-29-13-19920},
doi = {10.1364/OE.427247},
}

@article{Keldish:1965,
  title={ZhETF 47 1515 Google Scholar Keldysh LV 1965},
  author={Keldysh, LP},
  journal={Sov. Phys., JETP},
  volume={20},
  pages={235},
  year={1964}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%% DETECTORS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@article{Sizov:2018,
	doi = {10.1088/1361-6641/aae473},
	url = {https://doi.org/10.1088/1361-6641/aae473},
	year = 2018,
	month = {oct},
	publisher = {{IOP} Publishing},
	volume = {33},
	number = {12},
	pages = {123001},
	author = {F Sizov},
	title = {{Terahertz radiation detectors: the state-of-the-art}},
	journal = {Semiconductor Science and Technology},
}

@article{Lewis:2019,
	doi = {10.1088/1361-6463/ab31d5},
	url = {https://doi.org/10.1088/1361-6463/ab31d5},
	year = 2019,
	month = {aug},
	publisher = {{IOP} Publishing},
	volume = {52},
	number = {43},
	pages = {433001},
	author = {R A Lewis},
	title = {{A review of terahertz detectors}},
	journal = {Journal of Physics D: Applied Physics},
}

@article{TDStutorial:2018,
author = {Neu,Jens  and Schmuttenmaer,Charles A. },
title = {{Tutorial: An introduction to terahertz time domain spectroscopy (THz-TDS)}},
journal = {Journal of Applied Physics},
volume = {124},
number = {23},
pages = {231101},
year = {2018},
doi = {10.1063/1.5047659},
URL = {https://doi.org/10.1063/1.5047659},
eprint = {https://doi.org/10.1063/1.5047659}
}

@article{ABCD_Matsubara:2013,
author = {Eiichi Matsubara and Masaya Nagai and Masaaki Ashida},
journal = {J. Opt. Soc. Am. B},
number = {6},
pages = {1627--1630},
publisher = {OSA},
title = {{Coherent infrared spectroscopy system from terahertz to near infrared using air plasma produced by 10-fs pulses}},
volume = {30},
month = {Jun},
year = {2013},
url = {http://josab.osa.org/abstract.cfm?URI=josab-30-6-1627},
doi = {10.1364/JOSAB.30.001627},
}

@incollection{Wilke:2008,
  author      = {Ingrid Wilke and  Suranjana Sengupta},
  title       = {{Nonlinear Optical Techniques for Terahertz Pulse Generation and Detection -  Optical Rectification and Electrooptic Sampling}},
  editor      = {Susan L. Dexheimer},
  booktitle   = {Terahertz Spectroscopy: Principles and Applications},
  publisher   = {CRC Press},
  address     = {Boca Raton},
  year        = {2008},
  pages       = {41--72},
  chapter     = {2},
  url = {https://doi.org/10.1201/9781420007701},
}

@Article{OC_THzPhotonics:2019,
AUTHOR = {Jazbinsek, Mojca and Puc, Uros and Abina, Andreja and Zidansek, Aleksander},
TITLE = {{Organic Crystals for THz Photonics}},
JOURNAL = {Applied Sciences},
VOLUME = {9},
YEAR = {2019},
NUMBER = {5},
ARTICLE-NUMBER = {882},
URL = {https://www.mdpi.com/2076-3417/9/5/882},
ISSN = {2076-3417},
DOI = {10.3390/app9050882}
}

@article{Casalbuoni:2008,
  title = {{Numerical studies on the electro-optic detection of femtosecond electron bunches}},
  author = {Casalbuoni, S. and Schlarb, H. and Schmidt, B. and Schm\"user, P. and Steffen, B. and Winter, A.},
  journal = {Phys. Rev. ST Accel. Beams},
  volume = {11},
  issue = {7},
  pages = {072802},
  numpages = {18},
  year = {2008},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevSTAB.11.072802},
  url = {https://link.aps.org/doi/10.1103/PhysRevSTAB.11.072802}
}

@article{PlankenOrientation:2001,
author = {Paul C. M. Planken and Han-Kwang Nienhuys and Huib J. Bakker and Tom Wenckebach},
journal = {J. Opt. Soc. Am. B},
number = {3},
pages = {313--317},
publisher = {OSA},
title = {{Measurement and calculation of the orientation dependence of terahertz pulse detection in ZnTe}},
volume = {18},
month = {Mar},
year = {2001},
url = {http://josab.osa.org/abstract.cfm?URI=josab-18-3-313},
doi = {10.1364/JOSAB.18.000313},
}

@article{CLength:1996,
author = {Nahata,Ajay  and Weling,Aniruddha S.  and Heinz,Tony F. },
title = {{A wideband coherent terahertz spectroscopy system using optical rectification and electro-optic sampling}},
journal = {Applied Physics Letters},
volume = {69},
number = {16},
pages = {2321-2323},
year = {1996},
doi = {10.1063/1.117511},
URL = {https://doi.org/10.1063/1.117511},
}

@article{EOCs:1996,
author = {Wu,Q.  and Zhang,X.-C. },
title = {{Ultrafast electro-optic field sensors}},
journal = {Applied Physics Letters},
volume = {68},
number = {12},
pages = {1604-1606},
year = {1996},
doi = {10.1063/1.115665},
URL = {https://doi.org/10.1063/1.115665},
}

@article{Andriukaitis:2011,
author = {Giedrius Andriukaitis and Tadas Bal\v{c}i\={u}nas and Skirmantas Ali\v{s}auskas and Audrius Pug\v{z}lys and Andrius Baltu\v{s}ka and Tenio Popmintchev and Ming-Chang Chen and Margaret M. Murnane and Henry C. Kapteyn},
journal = {Opt. Lett.},
keywords = {Parametric oscillators and amplifiers; Ultrafast nonlinear optics; Laser materials; Optical amplifiers; Phase conjugation; Phase matching; Regenerative amplification; Strong field physics},
number = {15},
pages = {2755--2757},
publisher = {OSA},
title = {{90 GW peak power few-cycle mid-infrared pulses from an optical parametric amplifier}},
volume = {36},
month = {Aug},
year = {2011},
url = {http://ol.osa.org/abstract.cfm?URI=ol-36-15-2755},
doi = {10.1364/OL.36.002755},
}

@article{Shumakova:2018,
author = {V. Shumakova and S. Ali\v{s}auskas and P. Malevich and C. Gollner and A. Baltu\v{s}ka and D. Kartashov and A. M. Zheltikov and A. V. Mitrofanov and A. A. Voronin and D. A. Sidorov-Biryukov and A. Pug\v{z}lys},
journal = {Opt. Lett.},
number = {9},
pages = {2185--2188},
publisher = {OSA},
title = {{Filamentation of mid-IR pulses in ambient air in the vicinity of molecular resonances}},
volume = {43},
month = {May},
year = {2018},
url = {http://ol.osa.org/abstract.cfm?URI=ol-43-9-2185},
doi = {10.1364/OL.43.002185},
}



@article{Leitenstorfer:1999,
author = {Leitenstorfer,A.  and Hunsche,S.  and Shah,J.  and Nuss,M. C.  and Knox,W. H. },
title = {{Detectors and sources for ultrabroadband electro-optic sampling: Experiment and theory}},
journal = {Applied Physics Letters},
volume = {74},
number = {11},
pages = {1516-1518},
year = {1999},
doi = {10.1063/1.123601},
URL = {https://doi.org/10.1063/1.123601},
}

@article{SchneiderOR:2006,
author = {Arno Schneider and Max Neis and Marcel Stillhart and Blanca Ruiz and Rizwan U. A. Khan and Peter G\"{u}nter},
journal = {J. Opt. Soc. Am. B},
number = {9},
pages = {1822--1835},
publisher = {OSA},
title = {{Generation of terahertz pulses through optical rectification in organic DAST crystals: theory and experiment}},
volume = {23},
month = {Sep},
year = {2006},
url = {http://josab.osa.org/abstract.cfm?URI=josab-23-9-1822},
doi = {10.1364/JOSAB.23.001822},
}

@article{EOStutorial:2018,
author = {Neu,Jens  and Schmuttenmaer,Charles A. },
title = {{Tutorial: An introduction to terahertz time domain spectroscopy (THz-TDS)}},
journal = {Journal of Applied Physics},
volume = {124},
number = {23},
pages = {231101},
year = {2018},
doi = {10.1063/1.5047659},
URL = {https://doi.org/10.1063/1.5047659},
}

@article{BakkerEOS:1998,
author = {H. J. Bakker and G. C. Cho and H. Kurz and Q. Wu and X.-C. Zhang},
journal = {J. Opt. Soc. Am. B},
keywords = {Infrared; Pulses; Ultrafast measurements; Ultrafast nonlinear optics; Propagation; Femtosecond pulses; Phase matching; Phase velocity; Pockels effect; Ti:sapphire lasers; Ultrashort pulses},
number = {6},
pages = {1795--1801},
publisher = {OSA},
title = {{Distortion of terahertz pulses in electro-optic sampling}},
volume = {15},
month = {Jun},
year = {1998},
url = {http://josab.osa.org/abstract.cfm?URI=josab-15-6-1795},
doi = {10.1364/JOSAB.15.001795},
}

@article{Reimann:2007,
	doi = {10.1088/0034-4885/70/10/r02},
	url = {https://doi.org/10.1088/0034-4885/70/10/r02},
	year = 2007,
	month = {sep},
	publisher = {{IOP} Publishing},
	volume = {70},
	number = {10},
	pages = {1597--1632},
	author = {Klaus Reimann},
	title = {{Table-top sources of ultrashort {THz} pulses}},
	journal = {Reports on Progress in Physics},
}

@article{OhKim:2014,
author = {Oh,T. I.  and Yoo,Y. J.  and You,Y. S.  and Kim,K. Y. },
title = {{Generation of strong terahertz fields exceeding 8 {MV/cm} at 1 {kHz} and real-time beam profiling}},
journal = {Applied Physics Letters},
volume = {105},
number = {4},
pages = {041103},
year = {2014},
doi = {10.1063/1.4891678},
URL = {https://doi.org/10.1063/1.4891678},
eprint = {https://doi.org/10.1063/1.4891678}
}

%%%%%%%%%%% OR %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@book{Geoffry:2014,
    author    = {Geoffrey New},
    title     = {{Introduction to Nonlinear Optics}},
    year      = {2014},
    publisher = {cambridge university press},
    address   = {New York}
}

@article{Franken:1961,
  title = {{Generation of Optical Harmonics}},
  author = {Franken, P. A. and Hill, A. E. and Peters, C. W. and Weinreich, G.},
  journal = {Phys. Rev. Lett.},
  volume = {7},
  issue = {4},
  pages = {118--119},
  numpages = {0},
  year = {1961},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.7.118},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.7.118}
}

@article{Ravi:2014,
author = {Koustuban Ravi and W. Ronny Huang and Sergio Carbajo and Xiaojun Wu and Franz K\"{a}rtner},
journal = {Opt. Express},
number = {17},
pages = {20239--20251},
publisher = {OSA},
title = {{Limitations to THz generation by optical rectification using tilted pulse fronts}},
volume = {22},
month = {Aug},
year = {2014},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-22-17-20239},
doi = {10.1364/OE.22.020239},
}

@article{MPA_OR_Hoffmann:2007,
author = {Matthias C. Hoffmann and Ka-Lo Yeh and J\'{a}nos Hebling and Keith A. Nelson},
journal = {Opt. Express},
number = {18},
pages = {11706--11713},
publisher = {OSA},
title = {{Efficient terahertz generation by optical rectification at 1035 nm}},
volume = {15},
month = {Sep},
year = {2007},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-15-18-11706},
doi = {10.1364/OE.15.011706},
}

@article{MPA_Polonyi:2016,
author = {Gy. Pol\'{o}nyi and B. Monoszlai and G. G\"{a}umann and E. J. Rohwer and G. Andriukaitis and T. Balciunas and A. Pugzlys and A. Baltuska and T. Feurer and J. Hebling and J. A. F\"{u}l\"{o}p},
journal = {Opt. Express},
number = {21},
pages = {23872--23882},
publisher = {OSA},
title = {{High-energy terahertz pulses from semiconductors pumped beyond the three-photon absorption edge}},
volume = {24},
month = {Oct},
year = {2016},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-24-21-23872},
doi = {10.1364/OE.24.023872},
}

%%%%%%%%%%%%%%%%%%%organic crystals%%%%%%%%%%%%%%

@book{organicCrystalsBook:2015, 
place={Cambridge}, 
title={{Organic Electro-Optics and Photonics: Molecules, Polymers, and Crystals}}, 
DOI={10.1017/CBO9781139043885}, 
publisher={Cambridge University Press}, 
author={Dalton, Larry R. and Günter, Peter and Jazbinsek, Mojca and Kwon, O-Pil and Sullivan, Philip A.}, 
year={2015}
}

@article{MacroMicro:1982,
  title = {{Relations between microscopic and macroscopic lowest-order optical nonlinearities of molecular crystals with one- or two-dimensional units}},
  author = {Zyss, J. and Oudar, J. L.},
  journal = {Phys. Rev. A},
  volume = {26},
  issue = {4},
  pages = {2028--2048},
  numpages = {0},
  year = {1982},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.26.2028},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.26.2028}
}

@book{ocBookBosshard:1995, 
place={London}, 
title={{Organic Nonlinear Optical Materials}}, 
DOI={https://doi.org/10.4324/9780429114090 }, 
publisher={CRC Press}, 
author={Ch. Bosshard and K. Sutter and Ph. Pr\^{e}tre and J. Hulliger and M. Fl\"{o}rsheimer and P. Kaatzand P. G\"{u}nter}, 
year={1995}
}

@Article{Jazbinsek:2008,
author={Jazbinsek, Mojca and Mutter, Lukas and Gunter, Peter},
journal={IEEE Journal of Selected Topics in Quantum Electronics}, 
title={{Photonic Applications With the Organic Nonlinear Optical Crystal DAST}}, 
year={2008},
volume={14},
number={5},
pages={1298-1311},
doi={10.1109/JSTQE.2008.921407},
}

@article{refInd_Pan:1996,
author = {Pan,F.  and Kn\"{o}pfle,G.  and Bosshard,Ch.  and Follonier,S.  and Spreiter,R.  and Wong,M. S.  and G\"{u}nter,P. },
title = {{Electro-optic properties of the organic salt 4-N,N-dimethylamino-4'-N'-methyl-stilbazolium tosylate}},
journal = {Applied Physics Letters},
volume = {69},
number = {1},
pages = {13-15},
year = {1996},
doi = {10.1063/1.118101},
URL = {https://doi.org/10.1063/1.118101},
eprint = {https://doi.org/10.1063/1.118101}
}

@article{Cunningham:2010,
author = {Paul D. Cunningham and L. Michael Hayden},
journal = {Opt. Express},
number = {23},
pages = {23620--23625},
publisher = {OSA},
title = {{Optical properties of DAST in the THz range}},
volume = {18},
month = {Nov},
year = {2010},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-18-23-23620},
doi = {10.1364/OE.18.023620},
}

@article {Marder:1989,
	author = {Marder, Seth R. and Perry, Joseph W. and Schaefer, William P.},
	title = {{Synthesis of Organic Salts with Large Second-Order Optical Nonlinearities}},
	volume = {245},
	number = {4918},
	pages = {626--628},
	year = {1989},
	doi = {10.1126/science.245.4918.626},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	URL = {https://science.sciencemag.org/content/245/4918/626},
	eprint = {https://science.sciencemag.org/content/245/4918/626.full.pdf},
	journal = {Science}
}

@article{CascadedVicario:2014,
  title = {{$\mathrm{GV}/\mathrm{m}$ Single-Cycle Terahertz Fields from a Laser-Driven Large-Size Partitioned Organic Crystal}},
  author = {Vicario, Carlo and Monoszlai, Balazs and Hauri, Christoph P.},
  journal = {Phys. Rev. Lett.},
  volume = {112},
  issue = {21},
  pages = {213901},
  numpages = {5},
  year = {2014},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.112.213901},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.112.213901}
}

@Article{DASTCao:2016,
author ={Cao, Lifeng and Teng, Bing and Xu, Degang and Zhao, Huaisong and Hao, Lun and Yao, Jianquan and Guo, Jianqin},
title  ={Growth{,} transmission{,} {Raman} spectrum and {THz} generation of {DAST} crystal},
journal  ={RSC Adv.},
year  ={2016},
volume  ={6},
issue  ={1030},
pages  ={101389-101394},
publisher  ={The Royal Society of Chemistry},
doi  ={10.1039/C6RA15393C},
url  ={http://dx.doi.org/10.1039/C6RA15393C},
}

@article{DAST_TransVicario:2015,
	doi = {10.1088/2040-8978/17/9/094005},
	url = {https://doi.org/10.1088%2F2040-8978%2F17%2F9%2F094005},
	year = 2015,
	month = {sep},
	publisher = {{IOP} Publishing},
	volume = {17},
	number = {9},
	pages = {094005},
	author = {C. Vicario and B. Monoszlai and G. Arisholm and C. P. Hauri},
	title = {Generation of 1.5-octave intense infrared pulses by nonlinear interactions in {DAST} crystal},
	journal = {Journal of Optics},
}

@article{Zhen_YuCompetingNL:2008,
doi = {10.1088/0256-307x/25/5/094},
year = 2008,
month = {may},
publisher = {{IOP} Publishing},
volume = {25},
number = {5},
pages = {1868--1870},
author = {Zhao Zhen-Yu and Hameau Sophie and Tignon J{\'{e}}r{\^{o}}me},
title = {{THz Generation by Optical Rectification and Competition with Other Nonlinear Processes}},
journal = {Chinese Physics Letters},
}

@article{GaSeDamage2:2014,
author = {Feng,Z.-S.  and Kang,Z.-H.  and Li,X.-M.  and Wang,Zeng-Bin  and Gao,J.-Y.  and Andreev,Yu. M.  and Atuchin,V. V.  and Kokh,K. A.  and Lanskii,G. V.  and Potekaev,A. I.  and Shaiduko,A. V.  and Svetlichnyi,V. A. },
title = {Impact of fs and ns pulses on {Indium} and {Sulfur} doped {Gallium} {Selenide} crystals},
journal = {AIP Advances},
volume = {4},
number = {3},
pages = {037104},
year = {2014},
doi = {10.1063/1.4868626},
URL = {https://doi.org/10.1063/1.4868626},
eprint = {https://doi.org/10.1063/1.4868626}
}

@article{MostafaReRate:2015,
author = {Mostafa Shalaby and Christoph P. Hauri},
journal = {Scientific Reports},
pages = {8059--8063},
title = {Spectrally intense terahertz source based on triangular {Selenium}},
volume = {5},
month = {January},
year = {2015},
url = {https://doi.org/10.1038/srep08059},
doi = {10.1038/srep08059},
}

@article{RepRate:2013,
author = {Matsukawa,Takeshi  and Nawata,Kouji  and Notake,Takashi  and Qi,Feng  and 
Kawamata,Hiroshi  and Minamide,Hiroaki },
title = {{Pump-beam-induced optical damage depended on repetition frequency and pulse width in 4-dimethylamino-N-methyl-4-stilbazolium tosylate crystal}},
journal = {Applied Physics Letters},
volume = {103},
number = {2},
pages = {023302},
year = {2013},
doi = {10.1063/1.4813602},
URL = {https://doi.org/10.1063/1.4813602},
}

@article{2umLaser:2018,
author = {Xiaoming Ren and Lam H. Mach and Yanchun Yin and Yang Wang and Zenghu Chang},
journal = {Opt. Lett.},
keywords = {Infrared and far-infrared lasers; Rare earth and transition metal solid-state lasers; Ultrafast lasers; Laser amplifiers; Laser sources; Optical parametric chirped pulse amplification; Pulse compression; Q switched lasers; Strong field physics},
number = {14},
pages = {3381--3384},
publisher = {OSA},
title = {Generation of 1 {kHz}, 2.3 {mJ}, 88 fs, 2.5 $\mu\mathrm{m}$ pulses from a {$\mathrm{Cr^{2+}}$:ZnSe} chirped pulse amplifier },
volume = {43},
month = {Jul},
year = {2018},
url = {http://ol.osa.org/abstract.cfm?URI=ol-43-14-3381},
doi = {10.1364/OL.43.003381},
}

%%%%%%%%%%%%%%%%%%%%%%%%%% MID cohernce lengt %%%%%%%%%%%%%%%%%%%%
@article{InfraredBosshard:2002,
  title = {{Infrared and Raman spectroscopy of the organic crystal DAST: Polarization dependence and contribution of molecular vibrations to the linear electro-optic effect}},
  author = {Bosshard, Ch. and Spreiter, R. and Degiorgi, L. and G\"unter, P.},
  journal = {Phys. Rev. B},
  volume = {66},
  issue = {20},
  pages = {205107},
  numpages = {9},
  year = {2002},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.66.205107},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.66.205107}
}

@article{Stillhart:2008,
author = {Marcel Stillhart and Arno Schneider and Peter G\"{u}nter},
journal = {J. Opt. Soc. Am. B},
number = {11},
pages = {1914--1919},
publisher = {OSA},
title = {{Optical properties of 4-N,N-dimethylamino-4$\prime$-N$\prime$-methyl-stilbazolium 2,4,6-trimethylbenzenesulfonate crystals at terahertz frequencies}},
volume = {25},
month = {Nov},
year = {2008},
url = {http://josab.osa.org/abstract.cfm?URI=josab-25-11-1914},
doi = {10.1364/JOSAB.25.001914},
}

@article{Brunner:2008,
author = {Fabian D. J. Brunner and O-Pil Kwon and Seong-Ji Kwon and Mojca Jazbin\v{s}ek and Arno Schneider and Peter G\"{u}nter},
journal = {Opt. Express},
number = {21},
pages = {16496--16508},
publisher = {OSA},
title = {{A hydrogen-bonded organic nonlinear optical crystal for high-efficiency terahertz generation and detection}},
volume = {16},
month = {Oct},
year = {2008},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-16-21-16496},
doi = {10.1364/OE.16.016496},
}

@article{Pan1996CrystalGA,
  title={{Crystal growth and characterization of the organic salt 4-N, N-dimethylamino-42-N-methyl-stilbazolium tosylate (DAST)}},
  author={F. Pan and M. Wong and C. Bosshard and P. Guenter},
  journal={Advanced Materials},
  year={1996},
  volume={8},
  pages={592-595}
}

@article{Vodopyanov:2006,
author = {Konstantin L. Vodopyanov},
journal = {Opt. Express},
number = {6},
pages = {2263--2276},
publisher = {OSA},
title = {{Optical generation of narrow-band terahertz packets in periodically-inverted electro-optic crystals: conversion efficiency and optimal laser pulse format}},
volume = {14},
month = {Mar},
year = {2006},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-14-6-2263},
doi = {10.1364/OE.14.002263},
}

@article{PucGVD:2020,
author = {Puc, Uros and Bach, Tobias and Günter, Peter and Zgonik, Marko and Jazbinsek, Mojca},
title = {{Ultra-Broadband and High-Dynamic-Range THz Time-Domain Spectroscopy System Based on Organic Crystal Emitter and Detector in Transmission and Reflection Geometry}},
journal = {Advanced Photonics Research},
year={2020},
volume = {n/a},
number = {n/a},
pages = {2000098},
keywords = {DAST, DSTMS, organic crystals, reflections, spectroscopies, terahertz, transmissions},
doi = {https://doi.org/10.1002/adpr.202000098},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/adpr.202000098},
}

@article{Novelli:2020,
author = {Fabio Novelli and Biswajit Guchhait and Martina Havenith},
journal = {Materials (Basel)},
number = {6},
pages = {1311},
title = {{Towards Intense {THz} Spectroscopy on Water: Characterization of Optical Rectification by {GaP}, {OH1}, and {DSTMS} at {OPA} Wavelengths}},
volume = {13},
month = {March},
year = {2020},
url = {https://pubmed.ncbi.nlm.nih.gov/32183131},
doi = {10.3390/ma13061311},
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Quantum Dots %%%%%%%%%%%%%%%%%
@ARTICLE{Kirchain:2008,
    author = {Kirchain, Randolph and Kimerling, Lionel},
    title = {{A roadmap for nanophotonics}},
    journal = {Nature Photonics},
    year = {2007},
    volume = {1},
    pages = {303-305},
    doi = {10.1038/nphoton.2007.84},
    url = {https://doi.org/10.1038/nphoton.2007.84},
}

@ARTICLE{OmodulatorReed:2010,
    author = {Reed, G. T. and Mashanovich, G. and Gardes, F. Y. and Thomson, D. J.},
    title = {{Silicon optical modulators}},
    journal = {Nature Photonics},
    year = {2010},
    volume = {4},
    pages = {518--526},
    doi = {10.1038/nphoton.2010.179},
    url = {https://doi.org/10.1038/nphoton.2010.179},
}

@ARTICLE{OmodulatorKuo:2005,
    author = {Kuo, Yu-Hsuan and Lee, Yong Kyu and Ge, Yangsi and Ren, Shen and Roth, Jonathan E. and Kamins, Theodore I. abd Miller, David A. B. and Harris, James S.},
    title = {{Strong quantum-confined Stark effect in germanium quantum-well structures on silicon}},
    journal = {Nature},
    year = {2005},
    volume = {437},
    pages = {1334--1336},
    doi = {10.1038/nature04204},
    url = {https://doi.org/10.1038/nature04204},
}

@article{EOM_QW_Chaisakul:2012,
author = {Papichaya Chaisakul and Delphine Marris-Morini and Mohamed-Sa\"{i}d Rouifed and Giovanni Isella and Daniel Chrastina and Jacopo Frigerio and Xavier Le Roux and Samson Edmond and Jean-Ren\'{e} Coudevylle and Laurent Vivien},
journal = {Opt. Express},
number = {3},
pages = {3219--3224},
publisher = {OSA},
title = {{23 GHz Ge/SiGe multiple quantum well electro-absorption modulator}},
volume = {20},
month = {Jan},
year = {2012},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-20-3-3219},
doi = {10.1364/OE.20.003219},
}

@article{EOM_QW_Fukano:2007,
author = {Hideki Fukano and Takayuki Yamanaka and Munehisa Tamura},
journal = {J. Lightwave Technol.},
keywords = {Extinction; Extinction ratios; Modulators; Oscillator strengths; Polarized light; Quantum wells},
number = {8},
pages = {1961--1969},
publisher = {OSA},
title = {{Design and Fabrication of Low-Driving-Voltage Electroabsorption Modulators Operating at 40 Gb/s}},
volume = {25},
month = {Aug},
year = {2007},
url = {http://jlt.osa.org/abstract.cfm?URI=jlt-25-8-1961},
}

@article{RF_Stepanenko:2019,
	doi = {10.1088/1742-6596/1145/1/012028},
	url = {https://doi.org/10.1088/1742-6596/1145/1/012028},
	year = 2019,
	month = {jan},
	publisher = {{IOP} Publishing},
	volume = {1145},
	pages = {012028},
	author = {M. Stepanenko and I. Kulinich and I. Yunusov},
	title = {{Optimization of {RF} electrodes for electro-optic modulator based on quantum-confined Stark effect}},
	journal = {Journal of Physics: Conference Series},
}

@article{THzCommunitication:2010,
author = {Federici,John  and Moeller,Lothar },
title = {{Review of terahertz and subterahertz wireless communications}},
journal = {Journal of Applied Physics},
volume = {107},
number = {11},
pages = {111101},
year = {2010},
doi = {10.1063/1.3386413},
URL = {https://doi.org/10.1063/1.3386413},
}

@article{GaAs_Hoffmann:2010,
author = {Hoffmann,M. C.  and Monozon,B. S.  and Livshits,D.  and Rafailov,E. U.  and Turchinovich,D. },
title = {{Terahertz electro-absorption effect enabling femtosecond all-optical switching in semiconductor quantum dots}},
journal = {Applied Physics Letters},
volume = {97},
number = {23},
pages = {231108},
year = {2010},
doi = {10.1063/1.3515909},
URL = {https://doi.org/10.1063/1.3515909},
}

@article{Pein:2017,
author = {Pein, Brandt C. and Chang, Wendi and Hwang, Harold Y. and Scherer, Jennifer and Coropceanu, Igor and Zhao, Xiaoguang and Zhang, Xin and Bulović, Vladimir and Bawendi, Moungi and Nelson, Keith A.},
title = {{Terahertz-Driven Luminescence and Colossal Stark Effect in CdSe–CdS Colloidal Quantum Dots}},
journal = {Nano Letters},
volume = {17},
number = {9},
pages = {5375-5380},
year = {2017},
doi = {10.1021/acs.nanolett.7b01837},
URL = {https://doi.org/10.1021/acs.nanolett.7b01837},
}

@article{Pein:2019,
author = {Pein, Brandt C. and Lee, Chee Kong and Shi, Liang and Shi, JiaoJian and Chang, Wendi and Hwang, Harold Y. and Scherer, Jennifer and Coropceanu, Igor and Zhao, Xiaoguang and Zhang, Xin and Bulović, Vladimir and Bawendi, Moungi G. and Willard, Adam P. and Nelson, Keith A.},
title = {{Terahertz-Driven Stark Spectroscopy of CdSe and CdSe–CdS Core–Shell Quantum Dots}},
journal = {Nano Letters},
volume = {19},
number = {11},
pages = {8125-8131},
year = {2019},
doi = {10.1021/acs.nanolett.9b03342},
URL = {https://doi.org/10.1021/acs.nanolett.9b03342},
}

@article{Pero_Walters:2018,
author = {Walters, G. and Wei, M. and Voznyy, O. and Quintero-Bermudez, R. and Kiani, A. and Smilgies, D.M. and Munir, R. and Amassian, A. and Hoogland, S. and Sargent, E.},
title = {{The quantum-confined Stark effect in layered hybrid perovskites mediated by orientational polarizability of confined dipoles}},
journal = {Nature Communications},
volume = {9},
number = {2041-1723},
pages = {4214},
year = {2018},
doi = {10.1038/s41467-018-06746-5},
URL = {https://doi.org/10.1038/s41467-018-06746-5},
}

@article{TA_Zhang:2016,
title = {{Understanding the features in the ultrafast transient absorption spectra of {CdSe} quantum dots}},
journal = {Chemical Physics},
volume = {481},
pages = {157-164},
year = {2016},
issn = {0301-0104},
doi = {https://doi.org/10.1016/j.chemphys.2016.08.027},
url = {https://www.sciencedirect.com/science/article/pii/S0301010416304001},
author = {Cheng Zhang and Thanh Nhut Do and Xuanwei Ong and Yinthai Chan and Howe-Siang Tan},
}

@article{Norris:1996,
  title={{Measurement and assignment of the size-dependent optical spectrum in {CdSe} quantum dots}},
  author={Norris and Bawendi},
  journal={Physical review. B, Condensed matter},
  year={1996},
  volume={53},
  pages={16338-16346},
}

@article{Brus:1983,
author = {Brus,L. E. },
title = {{A simple model for the ionization potential, electron affinity, and aqueous redox potentials of small semiconductor crystallites}},
journal = {The Journal of Chemical Physics},
volume = {79},
number = {11},
pages = {5566--5571},
year = {1983},
doi = {10.1063/1.445676},
URL = {https://doi.org/10.1063/1.445676},
eprint = {https://doi.org/10.1063/1.445676}
}

@article{Brus:1984,
author = {Brus,L. E. },
title = {{Electron-electron and electron-hole interactions in small semiconductor crystallites: The size dependence of the lowest excited electronic state}},
journal = {The Journal of Chemical Physics},
volume = {80},
number = {9},
pages = {4403--4409},
year = {1984},
doi = {10.1063/1.447218},
URL = {https://doi.org/10.1063/1.447218},
eprint = {https://doi.org/10.1063/1.447218}
}

@article{Lippens:1989,
  title = {{Calculation of the band gap for small CdS and ZnS crystallites}},
  author = {Lippens, P. E. and Lannoo, M.},
  journal = {Phys. Rev. B},
  volume = {39},
  issue = {15},
  pages = {10935--10942},
  numpages = {0},
  year = {1989},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.39.10935},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.39.10935}
}

@article{Delure:1993,
  title = {{Theoretical aspects of the luminescence of porous silicon}},
  author = {Delerue, C. and Allan, G. and Lannoo, M.},
  journal = {Phys. Rev. B},
  volume = {48},
  issue = {15},
  pages = {11024--11036},
  numpages = {0},
  year = {1993},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.48.11024},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.48.11024}
}

@article{Wang:1996,
  title = {{Pseudopotential calculations of nanoscale CdSe quantum dots}},
  author = {Wang, Lin-Wang and Zunger, Alex},
  journal = {Phys. Rev. B},
  volume = {53},
  issue = {15},
  pages = {9579--9582},
  numpages = {0},
  year = {1996},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.53.9579},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.53.9579}
}

@article{Wang:1998,
  title = {{Applicability of the $\mathbf{k}\ensuremath{\cdot}\mathbf{p}$ method to the electronic structure of quantum dots}},
  author = {Fu, Huaxiang and Wang, Lin-Wang and Zunger, Alex},
  journal = {Phys. Rev. B},
  volume = {57},
  issue = {16},
  pages = {9971--9987},
  numpages = {0},
  year = {1998},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.57.9971},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.57.9971}
}

@article{Caram:2014,
author = {Caram,Justin R.  and Zheng,Haibin  and Dahlberg,Peter D.  and Rolczynski,Brian S.  and Griffin,Graham B.  and Dolzhnikov,Dmitriy S.  and Talapin,Dmitri V.  and Engel,Gregory S. },
title = {{Exploring size and state dynamics in {CdSe} quantum dots using two-dimensional electronic spectroscopy}},
journal = {The Journal of Chemical Physics},
volume = {140},
number = {8},
pages = {084701},
year = {2014},
doi = {10.1063/1.4865832},
URL = {https://doi.org/10.1063/1.4865832},
}

@book{schmidNanotechnology:2008,
  title={{Nanotechnology: Volume 1: Principles and Fundamentals}},
  author={Schmid, G. and Krug, H. and Waser, R.},
  isbn={9783527317325},
  lccn={2008428763},
  series={Nanotechnology (VCH)},
  url={https://books.google.at/books?id=2zBQtQEACAAJ},
  year={2008},
  publisher={Wiley}
}

@Article{Mastria:2016,
author ={Mastria, R. and Rizzo, A.},
title  ={{Mastering heterostructured colloidal nanocrystal properties for light-emitting diodes and solar cells}},
journal  ={J. Mater. Chem. C},
year  ={2016},
volume  ={4},
issue  ={27},
pages  ={6430-6446},
publisher  ={The Royal Society of Chemistry},
doi  ={10.1039/C6TC01334A},
url  ={http://dx.doi.org/10.1039/C6TC01334A},
}
@article{BandOffsetSteiner:2008,
author = {Steiner, Dov and Dorfs, Dirk and Banin, Uri and Della Sala, Fabio and Manna, Liberato and Millo, Oded},
title = {{Determination of Band Offsets in Heterostructured Colloidal Nanorods Using Scanning Tunneling Spectroscopy}},
journal = {Nano Letters},
volume = {8},
number = {9},
pages = {2954-2958},
year = {2008},
doi = {10.1021/nl801848x},
URL = {https://doi.org/10.1021/nl801848x},
eprint = {https://doi.org/10.1021/nl801848x}
}

@article{CihanBandAlignment2:2013,
author = {Cihan, Ahmet Fatih and Kelestemur, Yusuf and Guzelturk, Burak and Yerli, Ozan and Kurum, Ulas and Yaglioglu, Halime Gul and Elmali, Ayhan and Demir, Hilmi Volkan},
title = {{Attractive versus Repulsive Excitonic Interactions of Colloidal Quantum Dots Control Blue- to Red-Shifting (and Non-shifting) Amplified Spontaneous Emission}},
journal = {The Journal of Physical Chemistry Letters},
volume = {4},
number = {23},
pages = {4146-4152},
year = {2013},
doi = {10.1021/jz402211m},
URL = {https://doi.org/10.1021/jz402211m},
}

@article{ASE_Dong:2013,
author = {Lin Dong and Abhilash Sugunan and Jun Hu and Sicheng Zhou and Shanghua Li and Sergei Popov and Muhammet S. Toprak and Ari T. Friberg and Mamoun Muhammed},
journal = {Appl. Opt.},
number = {1},
pages = {105--109},
publisher = {OSA},
title = {{Photoluminescence from quasi-type-{II} spherical {CdSe-CdS} core-shell quantum dots}},
volume = {52},
month = {Jan},
year = {2013},
url = {http://ao.osa.org/abstract.cfm?URI=ao-52-1-105},
doi = {10.1364/AO.52.000105},
}

@article{Annual_Klimov:2007,
author = {Klimov, Victor I.},
title = {{Spectral and Dynamical Properties of Multiexcitons in Semiconductor Nanocrystals}},
journal = {Annual Review of Physical Chemistry},
volume = {58},
number = {1},
pages = {635-673},
year = {2007},
doi = {10.1146/annurev.physchem.58.032806.104537},
note ={PMID: 17163837},
URL = {https://doi.org/10.1146/annurev.physchem.58.032806.104537},
eprint = {https://doi.org/10.1146/annurev.physchem.58.032806.104537}
}

@article{KlimovTypeII:2007,
author = {Piryatinski, Andrei and Ivanov, Sergei A. and Tretiak, Sergei and Klimov, Victor I.},
title = {{E}ffect of {Q}uantum and {D}ielectric {C}onfinement on the {E}xciton--{E}xciton {I}nteraction {E}nergy in {T}ype {II} {C}ore/{S}hell {S}emiconductor {N}anocrystals},
journal = {Nano Letters},
volume = {7},
number = {1},
pages = {108-115},
year = {2007},
doi = {10.1021/nl0622404},
note ={PMID: 17212448},
URL = {https://doi.org/10.1021/nl0622404},
eprint = {https://doi.org/10.1021/nl0622404}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%QCSE%%%%%%%%%%%%%%%%%%%%%%%%%
@article{Miller:1984,
  title = {{Band-Edge Electroabsorption in Quantum Well Structures: The Quantum-Confined Stark Effect}},
  author = {Miller, D. A. B. and Chemla, D. S. and Damen, T. C. and Gossard, A. C. and Wiegmann, W. and Wood, T. H. and Burrus, C. A.},
  journal = {Phys. Rev. Lett.},
  volume = {53},
  issue = {22},
  pages = {2173--2176},
  numpages = {0},
  year = {1984},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.53.2173},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.53.2173}
}

@article{Miller:1985,
  title = {{Electric field dependence of optical absorption near the band gap of quantum-well structures}},
  author = {Miller, D. A. B. and Chemla, D. S. and Damen, T. C. and Gossard, A. C. and Wiegmann, W. and Wood, T. H. and Burrus, C. A.},
  journal = {Phys. Rev. B},
  volume = {32},
  issue = {2},
  pages = {1043--1060},
  numpages = {0},
  year = {1985},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.32.1043},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.32.1043}
}

@article{Miller:1986,
  title = {{Relation between electroabsorption in bulk semiconductors and in quantum wells: The quantum-confined Franz-Keldysh effect}},
  author = {Miller, D. A. B. and Chemla, D. S. and Schmitt-Rink, S.},
  journal = {Phys. Rev. B},
  volume = {33},
  issue = {10},
  pages = {6976--6982},
  numpages = {0},
  year = {1986},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.33.6976},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.33.6976}
}

@article{IonizationField:1972,
  title = {{Toward a Unified Theory of Urbach's Rule and Exponential Absorption Edges}},
  author = {Dow, John D. and Redfield, David},
  journal = {Phys. Rev. B},
  volume = {5},
  issue = {2},
  pages = {594--610},
  numpages = {0},
  year = {1972},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.5.594},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.5.594}
}



@article{Miller:1989,
author = { S.   Schmitt-Rink  and  D.S.   Chemla  and  D.A.B.   Miller },
title = {{Linear and nonlinear optical properties of semiconductor quantum wells}},
journal = {Advances in Physics},
volume = {38},
number = {2},
pages = {89-188},
year  = {1989},
publisher = {Taylor & Francis},
doi = {10.1080/00018738900101102},
URL = {https://doi.org/10.1080/00018738900101102},
eprint = {https://doi.org/10.1080/00018738900101102}
}

@article {Matsuura:1986,
	Title = {{Subbands and excitons in a quantum well in an electric field}},
	Author = {Matsuura, M and Kamizato, T},
	DOI = {10.1103/physrevb.33.8385},
	Number = {12},
	Volume = {33},
	Month = {June},
	Year = {1986},
	Journal = {Phys. Rev. B},
	ISSN = {0163-1829},
	Pages = {8385--8389},
	URL = {https://doi.org/10.1103/physrevb.33.8385},
}

@article{Hiroshima:1986,
author = {Hiroshima,T.  and Lang,R. },
title = {{Well size dependence of Stark shifts for heavy-hole and light-hole levels in {GaAs/AlGaAs} quantum wells}},
journal = {Applied Physics Letters},
volume = {49},
number = {11},
pages = {639-641},
year = {1986},
doi = {10.1063/1.97065},
URL = {https://doi.org/10.1063/1.97065},
eprint = {https://doi.org/10.1063/1.97065}
}

@article{nandan2019wavefunction,
  title={{Wavefunction engineering of type-{I}/type-{II} excitons of CdSe/CdS core-shell quantum dots}},
  author={Nandan, Yashaswi and Mehata, Mohan Singh},
  journal={Scientific reports},
  volume={9},
  number={1},
  pages={1--11},
  year={2019},
  publisher={Nature Publishing Group}
}

@book{peter2010fundamentals,
  title={{Fundamentals of semiconductors: physics and materials properties}},
  author={Peter, YU and Cardona, Manuel},
  year={2010},
  publisher={Springer Science \& Business Media}
}

@article{velizhanin2016renormalization,
  title={{Renormalization of optical transition strengths in semiconductor nanoparticles due to band mixing}},
  author={Velizhanin, Kirill A},
  journal={Chemical Physics},
  volume={481},
  pages={165--176},
  year={2016},
  publisher={Elsevier}
}

@article{tyrrell2011effective,
  title={{Effective mass modeling of excitons in type-{II} quantum dot heterostructures}},
  author={Tyrrell, EJ and Smith, JM},
  journal={Physical Review B},
  volume={84},
  number={16},
  pages={165328},
  year={2011},
  publisher={APS}
}

@article{li2004first,
  title={{First principle study of core/shell structure quantum dots}},
  author={Li, Jingbo and Wang, Lin-Wang},
  journal={Applied physics letters},
  volume={84},
  number={18},
  pages={3648--3650},
  year={2004},
  publisher={American Institute of Physics}
}

@article{csahin2012reordering,
  title={{Reordering orbitals of semiconductor multi-shell quantum dot-quantum well heteronanocrystals}},
  author={{\c{S}}ahin, Mehmet and Nizamoglu, Sedat and Yerli, Ozan and Volkan Demir, Hilmi},
  journal={Journal of Applied Physics},
  volume={111},
  number={2},
  pages={023713},
  year={2012},
  publisher={American Institute of Physics}
}

@article{kane1958influence,
  title={{The influence of exchange on the effective mass formalism}},
  author={Kane, Evan O},
  journal={Journal of Physics and Chemistry of Solids},
  volume={6},
  number={2-3},
  pages={236--241},
  year={1958},
  publisher={Elsevier}
}

@article{efros1996band,
  title={{Band-edge exciton in quantum dots of semiconductors with a degenerate valence band: Dark and bright exciton states}},
  author={Efros, Al L and Rosen, M and Kuno, Masaru and Nirmal, Manoj and Norris, David J and Bawendi, M},
  journal={Physical Review B},
  volume={54},
  number={7},
  pages={4843},
  year={1996},
  publisher={APS}
}

@article{shabaev2012fine,
  title={{Fine structure of the band-edge excitons and trions in {C}d{S}e/{C}d{S} core/shell nanocrystals}},
  author={Shabaev, Andrew and Rodina, AV and Efros, Al L},
  journal={Physical Review B},
  volume={86},
  number={20},
  pages={205311},
  year={2012},
  publisher={APS}
}

@article{kayanuma1986wannier,
  title={{Wannier exciton in microcrystals}},
  author={Kayanuma, Y},
  journal={Solid state communications},
  volume={59},
  number={6},
  pages={405--408},
  year={1986},
  publisher={Elsevier}
}

@article{nazzal2009comparative,
  title={{Comparative theoretical study of the size dependent electronic and optical properties in {CdS} and {CdSe} spherical nanocrystals}},
  author={Nazzal, Amjad and Fu, Huaxiang},
  journal={Journal of Computational and Theoretical Nanoscience},
  volume={6},
  number={6},
  pages={1277--1289},
  year={2009},
  publisher={American Scientific Publishers}
}

@article{casas2017effect,
  title={{Effect of dielectric constant on emission of {CdSe} quantum dots}},
  author={Casas Esp{\'\i}nola, J and Hern{\'a}ndez Contreras, X},
  journal={Journal of Materials Science: Materials in Electronics},
  volume={28},
  number={10},
  year={2017}
}

@article{dielEffectZeiri:2019,
title = {{Dielectric environment effect on linear and nonlinear optical properties for {C}d{S}/{Z}n{S} core/shell quantum dots}},
journal = {Results in Physics},
volume = {15},
pages = {102661},
year = {2019},
issn = {2211-3797},
doi = {https://doi.org/10.1016/j.rinp.2019.102661},
url = {https://www.sciencedirect.com/science/article/pii/S2211379719322430},
author = {N. Zeiri and A. Naifar and S. {Abdi-Ben Nasrallah} and M. Said},
}

@article{liptay1960bestimmung,
  title={Die {B}estimmung von absoluten {\"{U}bergangsmomentrichtungen} und von {D}ipolmomenten angeregter {M}olek\"{u}le aus {M}essungen des elektrischen {D}ichroismus. I. {T}heorie},
  author={Liptay, W and Czekalla, J},
  journal={Z. Naturforsch. A},
  volume={15},
  number={12},
  pages={1072--1079},
  year={1960},
  publisher={Verlag der Zeitschrift f{\"u}r Naturforschung}
}

@article{liptay1976optical,
  title={{Optical absorption of molecules in liquid solutions in an applied external electric field (electrochromism)}},
  author={Liptay, Wolfgang},
  journal={Ber. Bunsenges. Phys. Chem.},
  volume={80},
  number={3},
  pages={207--217},
  year={1976},
  publisher={Wiley Online Library}
}

@article{Liptay:1969,
author = {Liptay, W.},
title = {{Electrochromism and Solvatochromism}},
journal = {Angew. Chem. Int. Ed.},
volume = {8},
number = {3},
pages = {177-188},
keywords = {Electrochromism, Solvatochromism},
doi = {https://doi.org/10.1002/anie.196901771},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/anie.196901771},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/anie.196901771},
year = {1969}
}
%%%%%%%%%%%%%%%%% QD Paper%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@article{Chen:2013,
author = {Chen, Ou and Zhao, Jing and Chauhan, Vikash P. and Cui, Jian and Wong, Cliff and Harris, Daniel K. and Wei, He and Han, Hee-Sun and Fukumura, Dai and Jain, Rakesh K. and Bawendi, Moungi G.
},
title = {{Compact high-quality {CdS/CdS} core/shell nanocrystals with narrow emission linewidths and suppressed blinking}},
journal = {Nature Materials},
volume = {12},
number = {1476-4660},
pages = {445--451},
year = {2013},
doi = {10.1038/nmat3539},
URL = {https://doi.org/10.1038/nmat3539},
}

@article{Jasieniak:2009,
author = {Jasieniak, Jacek and Smith, Lisa and van Embden, Joel and Mulvaney, Paul and Califano, Marco},
title = {Re-examination of the {S}ize-{D}ependent {A}bsorption {P}roperties of {CdSe} {Q}uantum {D}ots},
journal = {The Journal of Physical Chemistry C},
volume = {113},
number = {45},
pages = {19468-19474},
year = {2009},
doi = {10.1021/jp906827m},
URL = {https://doi.org/10.1021/jp906827m},
eprint = {https://doi.org/10.1021/jp906827m}
}

@article{dielConstGrinolds:2015,
author = {Grinolds, Darcy D. W. and Brown, Patrick R. and Harris, Daniel K. and Bulovic, Vladimir and Bawendi, Moungi G.},
title = {{Quantum-Dot Size and Thin-Film Dielectric Constant: Precision Measurement and Disparity with Simple Models}},
journal = {Nano Letters},
volume = {15},
number = {1},
pages = {21-26},
year = {2015},
doi = {10.1021/nl5024244},
note ={PMID: 25531164},
URL = {https://doi.org/10.1021/nl5024244},
eprint = {https://doi.org/10.1021/nl5024244}
}

@article{dielConstVahdani:2014,
title = {{The effect of the electronic intersubband transitions of quantum dots on the linear and nonlinear optical properties of dot-matrix system}},
journal = {Superlattices and Microstructures},
volume = {76},
pages = {326-338},
year = {2014},
issn = {0749-6036},
doi = {https://doi.org/10.1016/j.spmi.2014.09.023},
url = {https://www.sciencedirect.com/science/article/pii/S0749603614003504},
author = {M.R.K. Vahdani},
}

@article{Garnet_Brugg:1981,
author = {G. A. Niklasson and C. G. Granqvist and O. Hunderi},
journal = {Appl. Opt.},
keywords = {Effective medium theory; Electromagnetic radiation; Forward scattering; Optical properties; Scattering theory; Solar energy},
number = {1},
pages = {26--30},
publisher = {OSA},
title = {{Effective medium models for the optical properties of inhomogeneous materials}},
volume = {20},
month = {Jan},
year = {1981},
url = {http://ao.osa.org/abstract.cfm?URI=ao-20-1-26},
doi = {10.1364/AO.20.000026},
}

@article{Bozy:2013,
author = {Bozyigit, Deniz and Yarema, Olesya and Wood, Vanessa},
title = {{Origins of Low Quantum Efficiencies in Quantum Dot {LED}s}},
journal = {Advanced Functional Materials},
volume = {23},
number = {24},
pages = {3024-3029},
doi = {https://doi.org/10.1002/adfm.201203191},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/adfm.201203191},
year = {2013}
}

@article {ASE1_Klimov:2000,
	author = {Klimov, V. I. and Mikhailovsky, A. A. and Xu, Su and Malko, A. and Hollingsworth, J. A. and Leatherdale, C. A. and Eisler, H.-J. and Bawendi, M. G.},
	title = {{Optical Gain and Stimulated Emission in Nanocrystal Quantum Dots}},
	volume = {290},
	number = {5490},
	pages = {314--317},
	year = {2000},
	doi = {10.1126/science.290.5490.314},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	URL = {https://science.sciencemag.org/content/290/5490/314},
	eprint = {https://science.sciencemag.org/content/290/5490/314.full.pdf},
	journal = {Science}
}

@article{ASE2_GiantRod:2018,
author = {Polovitsyn, Anatolii and Khan, Ali Hossain and Angeloni, Ilaria and Grim, Joel Q. and Planelles, Josep and Climente, Juan I. and Moreels, Iwan},
title = {{Synthesis of Anisotropic CdSe/CdS Dot-in-Giant-Rod Nanocrystals with Persistent Blue-Shifted Biexciton Emission}},
journal = {ACS Photonics},
volume = {5},
number = {11},
pages = {4561-4568},
year = {2018},
doi = {10.1021/acsphotonics.8b01028},
URL = {https://doi.org/10.1021/acsphotonics.8b01028},
eprint = {https://doi.org/10.1021/acsphotonics.8b01028}
}

@article{Gollner:2015,
author = {Gollner, Claudia and Ziegler, Johannes and Protesescu, Loredana and Dirin, Dmitry N. and Lechner, Rainer T. and Fritz-Popovski, Gerhard and Sytnyk, Mykhailo and Yakunin, Sergii and Rotter, Stefan and Yousefi Amin, Amir Abbas and Vidal, Cynthia and Hrelescu, Calin and Klar, Thomas A. and Kovalenko, Maksym V. and Heiss, Wolfgang},
title = {{Random Lasing with Systematic Threshold Behavior in Films of CdSe/CdS Core/Thick-Shell Colloidal Quantum Dots}},
journal = {ACS Nano},
volume = {9},
number = {10},
pages = {9792-9801},
year = {2015},
doi = {10.1021/acsnano.5b02739},
note ={PMID: 26364796},
URL = {https://doi.org/10.1021/acsnano.5b02739},
eprint = {https://doi.org/10.1021/acsnano.5b02739}
}

@article{BoxCar:2020,
author = {Khatua,Durga Prasad  and Gurung,Sabina  and Singh,Asha  and Khan,Salahuddin  and Sharma,Tarun Kumar  and Jayabalan,J. },
title = {{Filtering noise in time and frequency domain for ultrafast pump-probe performed using low repetition rate lasers}},
journal = {Review of Scientific Instruments},
volume = {91},
number = {10},
pages = {103901},
year = {2020},
doi = {10.1063/5.0010449},
URL = {https://doi.org/10.1063/5.0010449}
}

@article{CdS_StarkColvin:1994,
author = {Colvin,V. L.  and Cunningham,K. L.  and Alivisatos,A. P. },
title = {{Electric field modulation studies of optical absorption in CdSe nanocrystals: Dipolar character of the excited state}},
journal = {The Journal of Chemical Physics},
volume = {101},
number = {8},
pages = {7122-7138},
year = {1994},
doi = {10.1063/1.468338},
URL = {https://doi.org/10.1063/1.468338},
}

@article{Quenching:2007,
author = {Huang, Hao and Dorn, August and Nair, Gautham P. and Bulović, Vladimir and Bawendi, Moungi G.},
title = {{Bias-Induced Photoluminescence Quenching of Single Colloidal Quantum Dots Embedded in Organic Semiconductors}},
journal = {Nano Letters},
volume = {7},
number = {12},
pages = {3781-3786},
year = {2007},
doi = {10.1021/nl072263y},
note ={PMID: 18034504},
URL = {https://doi.org/10.1021/nl072263y},
eprint = {https://doi.org/10.1021/nl072263y}
}

@article{Quenching:2009,
author = {Jing,Pengtao  and Zheng,Jinju  and Zeng,Qinghui  and Zhang,Youlin  and Liu,Xiaomin  and Liu,Xueyan  and Kong,Xianggui  and Zhao,Jialong },
title = {{Shell-dependent electroluminescence from colloidal {CdSe} quantum dots in multilayer light-emitting diodes}},
journal = {Journal of Applied Physics},
volume = {105},
number = {4},
pages = {044313},
year = {2009},
doi = {10.1063/1.3079475},
URL = {https://doi.org/10.1063/1.3079475},
eprint = {https://doi.org/10.1063/1.3079475}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 2 Color THz generation%%%%%%%%%%%%
@article{Nguyen:2017,
author = {A. Nguyen and P. Gonz\'{a}lez de Alaiza Mart\'{i}nez and J. D\'{e}chard and I. Thiele and I. Babushkin and S. Skupin and L. Berg\'{e}},
journal = {Opt. Express},
number = {5},
pages = {4720--4740},
publisher = {OSA},
title = {{Spectral dynamics of THz pulses generated by two-color laser filaments in air: the role of Kerr nonlinearities and pump wavelength}},
volume = {25},
month = {Mar},
year = {2017},
url = {http://www.osapublishing.org/oe/abstract.cfm?URI=oe-25-5-4720},
doi = {10.1364/OE.25.004720},
}

@article{Berge:2013,
  title = {{3D Numerical Simulations of THz Generation by Two-Color Laser Filaments}},
  author = {Berg\'e, Luc and Skupin, Stefan and K\"ohler, Christian and Babushkin, Ihar and Herrmann, Joachim},
  journal = {Phys. Rev. Lett.},
  volume = {110},
  issue = {7},
  pages = {073901},
  numpages = {5},
  year = {2013},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.110.073901},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.110.073901}
}
@article{Fedorov:2018,
  title = {{Extreme THz fields from two-color filamentation of midinfrared laser pulses}},
  author = {Fedorov, Vladimir Yu. and Tzortzakis, Stelios},
  journal = {Phys. Rev. A},
  volume = {97},
  issue = {6},
  pages = {063842},
  numpages = {6},
  year = {2018},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.97.063842},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.97.063842}
}

@article{Nguyen:2018,
  title = {{Broadband terahertz radiation from two-color mid- and far-infrared laser filaments in air}},
  author = {Nguyen, Alis\'ee and Gonz\'alez de Alaiza Mart\'{\i}nez, Pedro and Thiele, Illia and Skupin, Stefan and Berg\'e, Luc},
  journal = {Phys. Rev. A},
  volume = {97},
  issue = {6},
  pages = {063839},
  numpages = {5},
  year = {2018},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.97.063839},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.97.063839}
}

@article{Cook:2000,
author = {D. J. Cook and R. M. Hochstrasser},
journal = {Opt. Lett.},
keywords = {Nonlinear optics, four-wave mixing; Infrared, far; Ultrafast nonlinear optics; Ultrafast technology},
number = {16},
pages = {1210--1212},
publisher = {OSA},
title = {{Intense terahertz pulses by four-wave rectification in air}},
volume = {25},
month = {Aug},
year = {2000},
url = {http://ol.osa.org/abstract.cfm?URI=ol-25-16-1210},
doi = {10.1364/OL.25.001210},
}

@article{Kim:2007,
author = {K. Y. Kim and J. H. Glownia and A. J. Taylor and G. Rodriguez},
journal = {Opt. Express},
keywords = {Photoionization; Spectroscopy, far infrared; Ultrafast phenomena; Plasmas},
number = {8},
pages = {4577--4584},
publisher = {OSA},
title = {{Terahertz emission from ultrafast ionizing air in symmetry-broken laser fields}},
volume = {15},
month = {Apr},
year = {2007},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-15-8-4577},
doi = {10.1364/OE.15.004577},
}

@ARTICLE{Kim:2009,
author = {K. Y. Kim},
title = {{Generation of coherent terahertz radiation in ultrafast laser-gas interactions}},
journal = {Physics of Plasmas},
year = {2009},
month = {may},
volume = {16},
number = {5},
eid = {056706},
pages = {056706},
doi = {10.1063/1.3134422},
adsurl = {http://adsabs.harvard.edu/abs/2009PhPl...16e6706K},
adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Fedorov:2017,
author={V Yu Fedorov and A D Koulouklidis and S Tzortzakis},
title={{THz generation by two-color femtosecond filaments with complex polarization states: four-wave mixing versus photocurrent contributions}},
journal={Plasma Physics and Controlled Fusion},
volume={59},
number={1},
pages={014025},
url={http://stacks.iop.org/0741-3335/59/i=1/a=014025},
year={2017},
}

@article{KimConical:2012,
  title = {{Off-Axis Phase-Matched Terahertz Emission from Two-Color Laser-Induced Plasma Filaments}},
  author = {You, Y. S. and Oh, T. I. and Kim, K. Y.},
  journal = {Phys. Rev. Lett.},
  volume = {109},
  issue = {18},
  pages = {183902},
  numpages = {5},
  year = {2012},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.109.183902},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.109.183902}
}

@article{Gorodetsky:2014,
  title = {{Physics of the conical broadband terahertz emission from two-color laser-induced plasma filaments}},
  author = {Gorodetsky, Andrei and Koulouklidis, Anastasios D. and Massaouti, Maria and Tzortzakis, Stelios},
  journal = {Phys. Rev. A},
  volume = {89},
  issue = {3},
  pages = {033838},
  numpages = {6},
  year = {2014},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.89.033838},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.89.033838}
}

@misc{fedorov2018generation,
      title={Generation of intense terahertz radiation by two-color filamentation of laser pulses with different wavelengths}, 
      author={Vladimir Yu. Fedorov and Stelios Tzortzakis},
      year={2018},
      eprint={1808.05804},
      archivePrefix={arXiv},
      primaryClass={physics.optics}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% in proceedings
@inproceedings{GaSeDamage1:2013,
author = {Jin Guo and Ji-Jiang Xie and Laiming Zhang and Fei Chen and Ke Jiang and Sergei V. Alexeev and Yury M. Andreev and Konstantin A. Kokh and Gregory V. Lanskii and Valery F. Losev and Dmitry M. Lubenko and Anna V. Shaiduko and Valeriy A. Svetlichnyi},
title = {{GaSe} damage threshold under {IR} pulse pumping },
volume = {8677},
booktitle = {{XIX International Symposium on High-Power Laser Systems and Applications 2012}},
editor = {Kerim R. Allakhverdiev},
organization = {International Society for Optics and Photonics},
publisher = {SPIE},
pages = {359 -- 366},
year = {2013},
doi = {10.1117/12.2008916},
URL = {https://doi.org/10.1117/12.2008916}
}

@inproceedings{Shumakova:2019,
author = {Valentina Shumakova and Claudia Gollner and Alexander Voronin and Alexander Mitrofanov and Dmitriy Sidorov-Biryukov and Aleksei Zheltikov and Daniil Kartashov and Andrius Baltuska and Audrius Pugzlys},
booktitle = {2019 Conference on Lasers and Electro-Optics Europe and European Quantum Electronics Conference},
journal = {2019 Conference on Lasers and Electro-Optics Europe and European Quantum Electronics Conference},
keywords = {Circular polarization; Harmonic generation; Light filaments; Photons; Raman scattering; Wave plates},
publisher = {Optical Society of America},
title = {{Comparative Study of Harmonic Generation in Air and Argon in Light Filaments Driven by Circularly Polarized mid-IR Pulses}},
year = {2019},
url = {http://www.osapublishing.org/abstract.cfm?URI=CLEO_Europe-2019-cd_1_1},
doi = {10.1364/CLEO_EUROPE.2019.cd_1_1}
}


@article{Thiele:2017,
  title = {{Broadband terahertz emission from two-color femtosecond-laser-induced microplasmas}},
  author = {Thiele, I. and Gonz\'alez de Alaiza Mart\'{\i}nez, P. and Nuter, R. and Nguyen, A. and Berg\'e, L. and Skupin, S.},
  journal = {Phys. Rev. A},
  volume = {96},
  issue = {5},
  pages = {053814},
  numpages = {11},
  year = {2017},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.96.053814},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.96.053814}
}


@ARTICLE{Kim:2012,
author={Kim, Ki-Yong and Glownia, James H. and Taylor, Antoinette J. and Rodriguez, George},
journal={IEEE Journal of Quantum Electronics}, 
title={{High-Power Broadband Terahertz Generation via Two-Color Photoionization in Gases}}, 
year={2012},
volume={48},
number={6},
pages={797-805},
doi={10.1109/JQE.2012.2190586}}

@article{You:2013,
author = {Yong Sing You and Taek Il Oh and Ki-Yong Kim},
journal = {Opt. Lett.},
number = {7},
pages = {1034--1036},
publisher = {OSA},
title = {{Mechanism of elliptically polarized terahertz generation in two-color laser filamentation}},
volume = {38},
month = {Apr},
year = {2013},
url = {http://www.osapublishing.org/ol/abstract.cfm?URI=ol-38-7-1034},
doi = {10.1364/OL.38.001034},
}

@article{Meng:2016,
author = {Meng,Chao  and Chen,Wenbo  and Wang,Xiaowei  and Lü,Zhihui  and Huang,Yindong  and Liu,Jinlei  and Zhang,Dongwen  and Zhao,Zengxiu  and Yuan,Jianmin },
title = {{Enhancement of terahertz radiation by using circularly polarized two-color laser fields}},
journal = {Applied Physics Letters},
volume = {109},
number = {13},
pages = {131105},
year = {2016},
doi = {10.1063/1.4963883},
URL = {https://doi.org/10.1063/1.4963883},
eprint = {https://doi.org/10.1063/1.4963883}
}

@article{Ionization:2006,
  title = {{Ultrafast ionization study of ${\mathrm{N}}_{2}$ in intense linearly and circularly polarized laser fields}},
  author = {McKenna, J. and Suresh, M. and Srigengan, B. and Williams, I. D. and Bryan, W. A. and English, E. M. L. and Stebbings, S. L. and Newell, W. R. and Turcu, I. C. E. and Smith, J. M. and Divall, E. J. and Hooker, C. J. and Langley, A. J. and Collier, J. L.},
  journal = {Phys. Rev. A},
  volume = {73},
  issue = {4},
  pages = {043401},
  numpages = {9},
  year = {2006},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.73.043401},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.73.043401}
}

@article{Zhang:2017_incommensurate,
author = {Lei Zhang and Guo-Li Wang and Song-Feng Zhao and Xiao-Xin Zhou},
title = {{Controlling of strong tunable THz emission with optimal incommensurate multi-color laser field}},
journal = {Physics of Plasmas},
volume = {24},
number = {2},
pages = {023116},
year = {2017},
doi = {10.1063/1.4976549},
URL = {http://dx.doi.org/10.1063/1.4976549},
eprint = {http://dx.doi.org/10.1063/1.4976549}
}

@article{Babushkin:2011,
  author={I Babushkin and S Skupin and A Husakou and C Köhler and E Cabrera-Granado and L Bergé and J Herrmann},
  title={{Tailoring terahertz radiation by controlling tunnel photoionization events in gases}},
  journal={New Journal of Physics},
  volume={13},
  number={12},
  pages={123029},
  url={http://stacks.iop.org/1367-2630/13/i=12/a=123029},
  year={2011}
}

@article{WangMIR:2011,
author = {Wei-Min Wang and Shigeo Kawata and Zheng-Ming Sheng and Yu-Tong Li and Li-Ming Chen and Lie-Jia Qian and Jie Zhang},
journal = {Opt. Lett.},
number = {14},
pages = {2608--2610},
publisher = {OSA},
title = {{Efficient terahertz emission by mid-infrared laser pulses from gas targets}},
volume = {36},
month = {Jul},
year = {2011},
url = {http://ol.osa.org/abstract.cfm?URI=ol-36-14-2608},
doi = {10.1364/OL.36.002608}
}

@article{MitrofanovHH:2015,
author = {Mitrofanov, A. V. and Voronin, A. A. and Sidorov-Biryukov, D. A. and Pug\v{z}lys, A. and Stepanov, E. A. and Andriukaitis, G. Fl\"{o}ry, T. and Ali\v{s}auskas, S. and Fedotov, A. B. and Baltu\v{s}ka, A. and Zheltikov, A. M.},
journal = {Scientific Reports},
number = {8368},
title = {{Mid-infrared laser filaments in the atmosphere}},
volume = {5},
month = {Feb},
year = {2015},
url = {https://doi.org/10.1038/srep08368},
doi = {10.1038/srep08368}
}

@article{Liu:2005,
author = {W. Liu and S.L. Chin},
journal = {Opt. Express},
keywords = {Pulse propagation and temporal solitons ; Self-focusing; Femtosecond lasers; High power lasers; Laser beams; Refractive index; Self phase modulation; White light},
number = {15},
pages = {5750--5755},
publisher = {OSA},
title = {{Direct measurement of the critical power of femtosecond Ti:sapphire laser pulse in air}},
volume = {13},
month = {Jul},
year = {2005},
url = {http://www.osapublishing.org/oe/abstract.cfm?URI=oe-13-15-5750},
doi = {10.1364/OPEX.13.005750},
}

@article{Kartashov:2013,
author = {D. Kartashov and S. Ali\v{s}auskas and A. Pug\v{z}lys and A. Voronin and A. Zheltikov and M. Petrarca and P. B\'{e}jot and J. Kasparian and J.-P. Wolf and A. Baltu\v{s}ka},
journal = {Opt. Lett.},
number = {16},
pages = {3194--3197},
publisher = {OSA},
title = {{Mid-infrared laser filamentation in molecular gases}},
volume = {38},
month = {Aug},
year = {2013},
url = {http://www.osapublishing.org/ol/abstract.cfm?URI=ol-38-16-3194},
doi = {10.1364/OL.38.003194},
}

@article{FedorovDisp:2020,
author = {Fedorov, Vladimir Yu. and Tzortzakis, Stelios},
journal = {Light: Science \& Applications},
number = {186},
title = {{Powerful terahertz waves from long-wavelength infrared laser filaments}},
volume = {9},
issue  ={1},
month = {Nov},
year = {2020},
url = {https://doi.org/10.1038/s41377-020-00423-3},
doi = {10.1038/s41377-020-00423-3},
}

@article{Tailliez,
	doi = {10.1088/1367-2630/abb863},
	url = {https://doi.org/10.1088/1367-2630/abb863},
	year = 2020,
	month = {oct},
	publisher = {{IOP} Publishing},
	volume = {22},
	number = {10},
	pages = {103038},
	author = {C Tailliez and A Stathopulos and S Skupin and D Buo{\v{z}}ius and I Babushkin and V Vai{\v{c}}aitis and L Berg{\'{e}}},
	title = {{Terahertz pulse generation by two-color laser fields with circular polarization}},
}

@article{FengGaSe:2014,
author = {Feng,Z.-S.  and Kang,Z.-H.  and Li,X.-M.  and Wang,Zeng-Bin  and Gao,J.-Y.  and Andreev,Yu. M.  and Atuchin,V. V.  and Kokh,K. A.  and Lanskii,G. V.  and Potekaev,A. I.  and Shaiduko,A. V.  and Svetlichnyi,V. A. },
title = {{Impact of fs and ns pulses on indium and sulfur doped gallium selenide crystals}},
journal = {AIP Advances},
volume = {4},
number = {3},
pages = {037104},
year = {2014},
doi = {10.1063/1.4868626},
URL = {https://doi.org/10.1063/1.4868626},
eprint = {https://doi.org/10.1063/1.4868626}
}

@article{TasosEfield:2016,
  title = {{Spectral bandwidth scaling laws and reconstruction of THz wave packets generated from two-color laser plasma filaments}},
  author = {Koulouklidis, A. D. and Fedorov, V. Yu. and Tzortzakis, S.},
  journal = {Phys. Rev. A},
  volume = {93},
  issue = {3},
  pages = {033844},
  numpages = {6},
  year = {2016},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.93.033844},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.93.033844}
}

@inproceedings{TasosFreeSpace:2020,
author = {A. D. Koulouklidis and V. Yu. Fedorov and C. Gollner and V. Shumakova and A. Pugžlys and A. Baltuška and S. Tzortzakis},
title = {{Free space broadband intense THz sources and applications}},
volume = {11390},
booktitle = {{Next-Generation Spectroscopic Technologies XIII}},
editor = {Luisa T.M. Profeta and Abul K. Azad and Steven M. Barnett},
organization = {International Society for Optics and Photonics},
publisher = {SPIE},
pages = {19 -- 34},
keywords = {Laser filamentation, Broadband THz, Strong field THz, Nonlinear THz},
year = {2020},
doi = {10.1117/12.2558454},
URL = {https://doi.org/10.1117/12.2558454}
}

@INPROCEEDINGS{TasosNL:2019,
author={Koulouklidis, Anastasios D. and Gollner, Claudia and Shumakova, Valentina and Fedorov, Vladimir Yu. and Pugžlys, Audrius and Baltuška, Andrius and Tzortzakis, Stelios},
booktitle={2019 44th International Conference on Infrared, Millimeter, and Terahertz Waves (IRMMW-THz)}, 
title={{Nonlinear THz Field Applications in Free Space}}, 
year={2019},
volume={},
number={},
pages={1-2},
doi={10.1109/IRMMW-THz.2019.8873709}}

@article{Kress:2004,
author = {Markus Kress and Torsten L\"{o}ffler and Susanne Eden and Mark Thomson and Hartmut G. Roskos},
journal = {Opt. Lett.},
number = {10},
pages = {1120--1122},
publisher = {OSA},
title = {{Terahertz-pulse generation by photoionization of air with laser pulses composed of both fundamental and second-harmonic waves}},
volume = {29},
month = {May},
year = {2004},
url = {http://www.osapublishing.org/ol/abstract.cfm?URI=ol-29-10-1120},
doi = {10.1364/OL.29.001120},
}

@article{AirCiddor:1996,
author = {Philip E. Ciddor},
journal = {Appl. Opt.},
number = {9},
pages = {1566--1573},
publisher = {OSA},
title = {Refractive index of air: new equations for the visible and near infrared},
volume = {35},
month = {Mar},
year = {1996},
url = {http://opg.optica.org/ao/abstract.cfm?URI=ao-35-9-1566},
doi = {10.1364/AO.35.001566},
}

@article{AirMathar:2007,
	doi = {10.1088/1464-4258/9/5/008},
	url = {https://doi.org/10.1088/1464-4258/9/5/008},
	year = 2007,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {9},
	number = {5},
	pages = {470--476},
	author = {Richard J Mathar},
	title = {Refractive index of humid air in the infrared: model fits},
	journal = {Journal of Optics A: Pure and Applied Optics},
}
%%%%%%%%%%%%%%%%%%%% XPM %%%%%%%%%%%%%%%%%%%%
@article{ShenXOM:2007,
  title = {{Nonlinear Cross-Phase Modulation with Intense Single-Cycle Terahertz Pulses}},
  author = {Shen, Y. and Watanabe, T. and Arena, D. A. and Kao, C.-C. and Murphy, J. B. and Tsang, T. Y. and Wang, X. J. and Carr, G. L.},
  journal = {Phys. Rev. Lett.},
  volume = {99},
  issue = {4},
  pages = {043901},
  numpages = {4},
  year = {2007},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.99.043901},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.99.043901}
}

@article{ShenXOM:2010,
  title = {{Electro-optic time lensing with an intense single-cycle terahertz pulse}},
  author = {Shen, Yuzhen and Carr, G. L. and Murphy, James B. and Tsang, Thomas Y. and Wang, Xijie and Yang, Xi},
  journal = {Phys. Rev. A},
  volume = {81},
  issue = {5},
  pages = {053835},
  numpages = {4},
  year = {2010},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.81.053835},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.81.053835}
}


@article{CaumesZnTe:2002,
  title = {{Kerr-Like Nonlinearity Induced via Terahertz Generation and the Electro-Optical Effect in Zinc Blende Crystals}},
  author = {Caumes, J-P. and Videau, L. and Rouyer, C. and Freysz, E.},
  journal = {Phys. Rev. Lett.},
  volume = {89},
  issue = {4},
  pages = {047401},
  numpages = {4},
  year = {2002},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.89.047401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.89.047401}
}
@article{VicarioXPM:2017,
  title = {{Subcycle Extreme Nonlinearities in GaP Induced by an Ultrastrong Terahertz Field}},
  author = {Vicario, Carlo and Shalaby, Mostafa and Hauri, Christoph P.},
  journal = {Phys. Rev. Lett.},
  volume = {118},
  issue = {8},
  pages = {083901},
  numpages = {5},
  year = {2017},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.118.083901},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.118.083901}
}

@article{Wu:1996,
author = {Wu,Q.  and Litz,M.  and Zhang,X.C. },
title = {{Broadband detection capability of ZnTe electro-optic field detectors}},
journal = {Applied Physics Letters},
volume = {68},
number = {21},
pages = {2924-2926},
year = {1996},
doi = {10.1063/1.116356},
URL = {https://doi.org/10.1063/1.116356},
eprint = {https://doi.org/10.1063/1.116356}
}

@article{HiroriPL:2011,
author = {Hirori, H. and Shinokita, K. and Shirai, M. and Tani, S. and Kadoya, Y. and Tanaka, K.},
title = {{Extraordinary carrier multiplication gated by a picosecond electric field pulse}},
journal = {Nature Communications},
volume = {2},
number = {594},
issue={1},
year = {2011},
doi = {10.1038/ncomms1598},
URL = {https://doi.org/10.1038/ncomms1598},
}

@article{WenPL:2008,
  title = {{Ultrafast electron cascades in semiconductors driven by intense femtosecond terahertz pulses}},
  author = {Wen, H. and Wiczer, M. and Lindenberg, A. M.},
  journal = {Phys. Rev. B},
  volume = {78},
  issue = {12},
  pages = {125203},
  numpages = {6},
  year = {2008},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.78.125203},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.78.125203}
}

@article{HiroriExciton:2010,
  title = {{Excitonic interactions with intense terahertz pulses in ZnSe/ZnMgSSe multiple quantum wells}},
  author = {Hirori, Hideki and Nagai, Masaya and Tanaka, Koichiro},
  journal = {Phys. Rev. B},
  volume = {81},
  issue = {8},
  pages = {081305},
  numpages = {4},
  year = {2010},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.81.081305},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.81.081305}
}

@article{Watanabe:2011,
author = {Shinichi Watanabe and Nobutsugu Minami and Ryo Shimano},
journal = {Opt. Express},
number = {2},
pages = {1528--1538},
publisher = {OSA},
title = {{Intense terahertz pulse induced exciton generation in carbon nanotubes}},
volume = {19},
month = {Jan},
year = {2011},
url = {http://www.osapublishing.org/oe/abstract.cfm?URI=oe-19-2-1528},
doi = {10.1364/OE.19.001528},
}


@article{Nordstrom:1998,
  title = {{Excitonic Dynamical Franz-Keldysh Effect}},
  author = {Nordstrom, K. B. and Johnsen, K. and Allen, S. J. and Jauho, A.-P. and Birnir, B. and Kono, J. and Noda, T. and Akiyama, H. and Sakaki, H.},
  journal = {Phys. Rev. Lett.},
  volume = {81},
  issue = {2},
  pages = {457--460},
  numpages = {0},
  year = {1998},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.81.457},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.81.457}
}

@article{PLshift:1987,
  title = {{Dimensionality dependence of the band-gap renormalization in two- and three-dimensional electron-hole plasmas in GaAs}},
  author = {Tr\"ankle, G. and Leier, H. and Forchel, A. and Haug, H. and Ell, C. and Weimann, G.},
  journal = {Phys. Rev. Lett.},
  volume = {58},
  issue = {4},
  pages = {419--422},
  numpages = {0},
  year = {1987},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.58.419},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.58.419}
}

@article{Kaindl:2009,
  title = {{Transient terahertz spectroscopy of excitons and unbound carriers in quasi-two-dimensional electron-hole gases}},
  author = {Kaindl, R. A. and H\"agele, D. and Carnahan, M. A. and Chemla, D. S.},
  journal = {Phys. Rev. B},
  volume = {79},
  issue = {4},
  pages = {045320},
  numpages = {13},
  year = {2009},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.79.045320},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.79.045320}
}

@article{KnifeEdge:2009,
author = {Marcos A. de Ara\'{u}jo and Rubens Silva and Emerson de Lima and Daniel P. Pereira and Paulo C. de Oliveira},
journal = {Appl. Opt.},
keywords = {Numerical approximation and analysis; Paraxial wave optics ; Metrology; Laser beam characterization ; Electric fields; Gaussian beams; Integrating spheres; Laser beam characterization; Laser beams; Z scanning},
number = {2},
pages = {393--396},
publisher = {OSA},
title = {Measurement of Gaussian laser beam radius using the knife-edge technique: improvement on data analysis},
volume = {48},
month = {Jan},
year = {2009},
url = {http://www.osapublishing.org/ao/abstract.cfm?URI=ao-48-2-393},
doi = {10.1364/AO.48.000393},
}

@article{Song:2021,
author = {Qiying Song and Xinming Yuan and Qinggang Lin and Haizhe Zhong and Xuanke Zeng and Yi Cai and Xiaowei Lu and Maijie Zheng and Wenhua Cao and Shixiang Xu},
journal = {Opt. Express},
keywords = {High harmonic generation; High power lasers; Laser energy; Laser filaments; Phase shift; Terahertz generation},
number = {26},
pages = {43379--43388},
publisher = {OSA},
title = {Experimentally exploring the terahertz radiation in a long filament by a two-color laser field},
volume = {29},
month = {Dec},
year = {2021},
url = {http://opg.optica.org/oe/abstract.cfm?URI=oe-29-26-43379},
doi = {10.1364/OE.439938},
}

@article{Auger:2015,
author = {Vaxenburg, Roman and Rodina, Anna and Shabaev, Andrew and Lifshitz, Efrat and Efros, Alexander L.},
title = {Nonradiative Auger Recombination in Semiconductor Nanocrystals},
journal = {Nano Letters},
volume = {15},
number = {3},
pages = {2092-2098},
year = {2015},
doi = {10.1021/nl504987h},
note ={PMID: 25693512},
URL = {https://doi.org/10.1021/nl504987h},
eprint = {https://doi.org/10.1021/nl504987h}
}

@book{chin_femtosecond:2010,
  title={Femtosecond laser filamentation},
  author={Chin, See Leang},
  volume={55},
  year={2010},
  publisher={Springer}
}

@article{Geints:2014,
	doi = {10.1070/qe2014v044n05abeh015427},
	url = {https://doi.org/10.1070/qe2014v044n05abeh015427},
	year = 2014,
	month = {may},
	publisher = {{IOP} Publishing},
	volume = {44},
	number = {5},
	pages = {489--497},
	author = {Yu E Geints and S S Golik and A A Zemlyanov and A M Kabanov and G G Matvienko},
	title = {Influence of the laser beam size on the length of a filament formed by high-power femtosecond laser radiation in air},
	journal = {Quantum Electronics},
}

@article{Marburger:1975,
title = {Self-focusing: Theory},
journal = {Progress in Quantum Electronics},
volume = {4},
pages = {35-110},
year = {1975},
issn = {0079-6727},
doi = {https://doi.org/10.1016/0079-6727(75)90003-8},
url = {https://www.sciencedirect.com/science/article/pii/0079672775900038},
author = {J.H. Marburger}
}

@article{Skupin:2007,
title = {Supercontinuum generation of ultrashort laser pulses in air at different central wavelengths},
journal = {Optics Communications},
volume = {280},
number = {1},
pages = {173-182},
year = {2007},
issn = {0030-4018},
doi = {https://doi.org/10.1016/j.optcom.2007.06.067},
url = {https://www.sciencedirect.com/science/article/pii/S0030401807006396},
author = {Stefan Skupin and Luc Berge},
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@incollection{Boyd:2003,
editor = {Robert W. Boyd},
booktitle = {{Nonlinear Optics (Second Edition)}},
publisher = {Academic Press},
edition = {Second Edition},
address = {San Diego},
pages = {xv-xvii},
year = {2003},
isbn = {978-0-12-121682-5},
doi = {https://doi.org/10.1016/B978-012121682-5/50001-8},
url = {https://www.sciencedirect.com/science/article/pii/B9780121216825500018}
}


%%%%%%%%%%%%%%%%%%%%%%%%%PhD Thesis
@phdthesis{PhDMutter:2007,
	Type = {dissertation},
	Title = {{Nonlinear optical organic crystals for photonic applications}},
	Author = {Lukas Muttre},
	School = {ETH Zurich},
	URL = {https://doi.org/10.3929/ethz-a-005521077},
 	Year = {2007}
} 

@phdthesis{Valentina:2018,
	Type = {dissertation},
	Title = {Filamentation and self-compression of multi-mJ fs mid-infrared pulses},
	Author = {Shumakova, Valentina},
	School = {TU Wien},
	URL = {https://permalink.catalogplus.tuwien.at/AC15077015},
 	Year = {2018}
} 

@mastersthesis{Daniel:2021,
	Type = {Bachelor's Thesis},
	Title = {{Numerical studies on THz pulse retrieval measured by electro-optical sampling with GaP}},
	Author = {Wendl, Daniel},
	School = {TU Wien},
 	Year = {2021},
}


